Estimating returns to special education: combining machine learning and text analysis to address confounding

Leveraging unique insights into the special education placement process through written individual psychological records, I present results from the first ever study to examine short- and long-term returns to special education programs with causal machine learning and computational text analysis methods. I find that special education programs in inclusive settings have positive returns in terms of academic performance as well as labor-market integration. Moreover, I uncover a positive effect of inclusive special education programs in comparison to segregated programs. This effect is heterogenous: segregation has least negative effects for students with emotional or behavioral problems, and for nonnative students with special needs. Finally, I deliver optimal program placement rules that would maximize aggregated school performance and labor market integration for students with special needs at lower program costs. These placement rules would reallocate most students with special needs from segregation to inclusion.

==> Tables/Archives/optimal.policy_May2021.tex <==
\begin{table}[p!]
\footnotesize
\centering
\begin{tabular}{lccccc}
\multicolumn{3}{l}{\textbf{Panel A}: Allocation to program in percent and potential cost reduction} \\[1ex]

  \toprule
                                &\% Students    &\% Students        &Policy           &Costs per year      & Percent of   \\ 
                                &sent to        &sent to semi-      &value            &(in mio CHF)        & actual costs   \\ 
                                &inclusion      &segregation        &                 &                    &  \\
  \midrule
\multicolumn{3}{l}{\emph{Test scores. N = 2988}} \\[1ex]
\textbf{Actual allocation}      &0.688          &0.312                &-0.581         &63,949           &1       \\
Depth 2 and baseline variables  &0.820          &0.180                &-0.353         &62,176           &0.972    \\
Depth 3 and baseline variables  &0.822          &0.178                &-0.262         &62,149           &0.972   \\
Depth 2 and diagnosis variables &0.820          &0.180                &-0.353         &62,176           &0.972   \\
Depth 3 and diagnosis variables &0.771          &0.229                &-0.249         &62,833           &0.983   \\[4ex]


\multicolumn{3}{l}{\emph{Probability to be employed. N = 2940}} \\[1ex]
\textbf{Actual allocation}      &0.533          &0.467                &0.408          &64,983           &1       \\
Depth 2 and baseline variables  &0.948          &0.052                &0.863          &59,493           &0.916   \\
Depth 3 and baseline variables  &0.873          &0.127                &0.928          &60,478           &0.931   \\
Depth 2 and diagnosis variables &0.930          &0.071                &0.890          &59,727           &0.919  \\
Depth 3 and diagnosis variables &0.836          &0.164                &0.956          &60,973           &0.938   \\
\bottomrule
\end{tabular}

\begin{comment}
\multicolumn{3}{l}{\emph{Overall welfare (50\% academic performance, 50\% labor market integration. N = 2940}} \\[1ex]
\textbf{Actual allocation }       &0.602        &0.398                &0.00393       &41,139          &1      \\
Depth 2 and baseline variables    &0.908        &0.0922               &0.0174        &38,543          &0.937  \\
Depth 3 and baseline variables    &0.826        &0.174                &0.0239        &39,240          &0.954  \\
Depth 2 and diagnosis variables   &0.908        &0.0922               &0.0174        &38,543          &0.937  \\
Depth 3 and diagnosis variables   &0.826        &0.174                &0.0239        &39,240          &0.954  \\
\end{comment}


\vspace{10mm}

\begin{tabular}{lccc}
\multicolumn{3}{l}{\textbf{Panel B}: Cross-validated difference between optimal policy value and different policies} \\[1ex]
\toprule
                                  & All inclusion           &All semi-segregation           &Assigned policy \\
\midrule
\multicolumn{3}{l}{\emph{Test scores. N = 2988}} \\[1ex]
Depth 2 and baseline variables    &-0.054                   &0.515$^{***}$                  &0.375$^{***}$   \\  
                                  &(0.04)                   &(0.12)                         &(0.07)        \\
Depth 3 and baseline variables    &-0.047                   &0.523$^{***}$                  &0.382$^{***}$   \\ 
                                  &(0.05)                   &(0.11)                         &(0.07)        \\
Depth 2 and diagnosis variables   &-0.093$^{*}$             &0.477$^{***}$                  &0.336$^{***}$   \\   
                                  &(0.05)                   &(0.11)                         &(0.07)        \\
Depth 3 and diagnosis variables   &-0.109$^{*}$             &0.461$^{***}$                  &0.320$^{***}$   \\   
                                  &(0.06)                   &(0.11)                         &(0.07)        \\[4ex]


\multicolumn{3}{l}{\emph{Probability to be employed. N = 2940}} \\[1ex]
Depth 2 and baseline variables    &0.042$^{*}$              &-0.482$^{***}$                 &-0.060     \\  
                                  &(0.02)                   &(0.11)                         &(0.05)       \\
Depth 3 and baseline variables    &0.107$^{*}$              &-0.417$^{***}$                 &0.045  \\ 
                                  &(0.06)                   &(0.1)                          &(0.07)        \\
Depth 2 and diagnosis variables   &0.042$^{*}$              &-0.483$^{***}$                 &-0.061  \\   
                                  &(0.02)                   &(0.11)                         &(0.05)        \\
Depth 3 and diagnosis variables   &0.001                    &-0.519$^{***}$                 &-0.097$^{*}$        \\   
                                  &(0.03)                   &(0.11)                         &(0.05)        \\

\bottomrule
& \multicolumn{3}{r}{\emph{Notes:}$^{***}$: p $<$0.01, $^{**}$: p $<$ 0.05, $^{*}$: p $<$ 0.1.} \\
& \multicolumn{3}{r}{Optimal policies computed on 10-fold cross validation.} \\[1ex]
\end{tabular}
\begin{comment}
Depth 2 and diagnosis variables  &-0.0159       &0.007$^{***}$        &0.004      \\
                                 &0.012         &(0.00)               &(0.01)     \\
Depth 3 and diagnosis variables  &-0.0138       &0.009$^{***}$        &0.006      \\
                                 &(0.011)       &(0.00)               &(0.01)     \\
Depth 2 and baseline variables   &-0.0188       &0.004$^{*}$          &0.001      \\
                                 &(0.0117)      &(0.00)               &(0.01)     \\
Depth 3 and baseline variables   &-0.0191$^{*}$ &0.004                &0.001      \\
                                 &(0.0116)      &(0.00)               &(0.01)     \\
\end{comment}

\caption{Optimal policies for inclusion and semi-segregation} 
\label{table:optimal_policy}
\end{table}

==> Tables/Archives/outcome.RMSE.old.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Fri Oct 23 00:28:40 2020
\begin{table}[h]
\centering
\begingroup\scriptsize
\begin{tabular}{llccc}
  \toprule
Outcome & Method & RMSE (mean) & RMSE (max) & RMSE (min) \\ 
  \midrule
Probability of using DI & Text tf and covariates, with RF & 0.229 & 0.233 & 0.225 \\ 
  Probability of using DI & STM, k = 80, with Lasso & 0.229 & 0.235 & 0.224 \\ 
  Probability of using DI & STM, k = 10, with RF & 0.231 & 0.235 & 0.224 \\ 
  Probability of using DI & STM, k = 80, with E.net & 0.229 & 0.235 & 0.224 \\ 
  Probability of using DI & Text tf.tf.idf and covariates, with RF & 0.229 & 0.233 & 0.226 \\ 
   \midrule
Probability of VET & STM, k = 10, with RF & 0.419 & 0.420 & 0.417 \\ 
  Probability of VET & Text tf.tf.idf and covariates, with RF & 0.419 & 0.420 & 0.418 \\ 
  Probability of VET & STM, k = 80, with Lasso & 0.419 & 0.420 & 0.419 \\ 
  Probability of VET & STM, k = 80, with E.net & 0.419 & 0.420 & 0.419 \\ 
  Probability of VET & Text tf.idf and covariates, with E.net & 0.420 & 0.421 & 0.420 \\ 
   \midrule
Probability of no education & STM, k = 80, with Lasso & 0.408 & 0.410 & 0.405 \\ 
  Probability of no education & STM, k = 80, with E.net & 0.408 & 0.410 & 0.405 \\ 
  Probability of no education & Text tf.tf.idf and covariates, with E.net & 0.410 & 0.411 & 0.408 \\ 
  Probability of no education & Text tf.tf.idf and covariates, with RF & 0.409 & 0.410 & 0.406 \\ 
  Probability of no education & Text tf.tf.idf and covariates, with Lasso & 0.410 & 0.411 & 0.408 \\ 
   \midrule
Work income & Text tf and covariates, with RF & 0.786 & 0.809 & 0.763 \\ 
  Work income & STM, k = 80, with E.net & 0.788 & 0.813 & 0.765 \\ 
  Work income & STM, k = 80, with Lasso & 0.788 & 0.813 & 0.765 \\ 
  Work income & Text tf.idf and covariates, with RF & 0.789 & 0.813 & 0.767 \\ 
  Work income & Word2Vec25, with RF & 0.789 & 0.814 & 0.766 \\ 
   \midrule
Probability to have minimum wage & STM, k = 80, with E.net & 0.430 & 0.435 & 0.426 \\ 
  Probability to have minimum wage & STM, k = 80, with Lasso & 0.430 & 0.435 & 0.426 \\ 
  Probability to have minimum wage & Text tf.idf and covariates, with Lasso & 0.431 & 0.435 & 0.427 \\ 
  Probability to have minimum wage & Text tf.idf and covariates, with E.net & 0.431 & 0.435 & 0.427 \\ 
  Probability to have minimum wage & Text tf.tf.idf and covariates, with Lasso & 0.431 & 0.435 & 0.427 \\ 
   \midrule
Probability of taking the SW8 test & STM, k = 80, with Lasso & 0.369 & 0.371 & 0.364 \\ 
  Probability of taking the SW8 test & Text tf.tf.idf and covariates, with RF & 0.367 & 0.371 & 0.364 \\ 
  Probability of taking the SW8 test & Text tf.idf and covariates, with RF & 0.369 & 0.372 & 0.366 \\ 
  Probability of taking the SW8 test & STM, k = 80, with E.net & 0.369 & 0.371 & 0.364 \\ 
  Probability of taking the SW8 test & STM, k = 10, with RF & 0.369 & 0.372 & 0.366 \\ 
   \midrule
SW8 test results & Text tf and covariates, with Lasso & 0.776 & 0.780 & 0.773 \\ 
  SW8 test results & Text tf and covariates, with E.net & 0.777 & 0.781 & 0.775 \\ 
  SW8 test results & Text tf.idf and covariates, with E.net & 0.780 & 0.781 & 0.778 \\ 
  SW8 test results & Text tf.idf and covariates, with Lasso & 0.781 & 0.786 & 0.778 \\ 
  SW8 test results & Word2Vec100, with Lasso & 0.783 & 0.788 & 0.780 \\ 
   \midrule
Probability of being unemployed & STM, k = 80, with Lasso & 0.414 & 0.417 & 0.410 \\ 
  Probability of being unemployed & Text tf and covariates, with E.net & 0.414 & 0.418 & 0.411 \\ 
  Probability of being unemployed & STM, k = 80, with E.net & 0.414 & 0.417 & 0.410 \\ 
  Probability of being unemployed & Word2Vec100, with Lasso & 0.414 & 0.417 & 0.411 \\ 
  Probability of being unemployed & Text tf.tf.idf and covariates, with Lasso & 0.414 & 0.417 & 0.411 \\ 
   \midrule
Work income (month) & Text tf and covariates, with RF & 0.956 & 0.979 & 0.936 \\ 
  Work income (month) & STM, k = 80, with Lasso & 0.956 & 0.978 & 0.938 \\ 
  Work income (month) & STM, k = 80, with E.net & 0.956 & 0.979 & 0.938 \\ 
  Work income (month) & STM, k = 10, with E.net & 0.960 & 0.979 & 0.946 \\ 
  Work income (month) & Word2Vec25, with RF & 0.959 & 0.981 & 0.942 \\ 
   \bottomrule 
 \multicolumn{5}{l}{\scriptsize{Mean, max and min RMSE for each text representation overthe different folds. The 5 methods with lowest RMSE are reported.}} 
\end{tabular}
\endgroup
\caption{Ensemble learner for outcome} 
\label{outcome.RMSE}
\end{table}


==> Tables/Archives/table_summary_stats_treatment.tex <==
\begin{table}
\centering
\scriptsize
\begin{tabular}{lccccc}
  \toprule
    & Inclusive special ed. (ISF) & Individual therapy  & No therapy        & Segr. small classes & Segregated schooling \\ 
    & (ISF)                       &                     & (but sent to SPS) &                     & \\
  \midrule
  $N$ ($N = 21343$)  &    2705 &    7992 &    7353 &    1690 &    1603 \\ 
  
  \addlinespace[1em]
  \multicolumn{5}{l}{\textbf{A: Individual characteristics}}\\
  Female                  &    0.46  &    0.40  &    0.40  &    0.43  &    0.30  \\ 
  Foreign language        &    0.11  &    0.09  &    0.09  &    0.28  &    0.14  \\ 
  IQ                      &   92.94 (9.41) &   98.27 (10.58) &   99.59 (13.50) &   86.17 (8.96) &   87.01 (14.99) \\ 
  IQ measured             &    0.80  &    0.74  &    0.45  &    0.78  &    0.67  \\ 
  Birth year              & 1996.68 (3.73) & 1995.14 (4.33) & 1993.88 (5.38) & 1993.61 (3.64) & 1995.80 (4.31) \\ 
  Age at first interview  &    8.75 (2.03) &    8.69 (1.96) &    9.04 (2.94) &    9.11 (2.50) &    7.19 (2.63) \\ 
  Had bridge year         &    0.07  &    0.08  &    0.17  &    0.13  &    0.08  \\ 
  Reasons: other          &    0.02  &    0.03  &    0.06  &    0.06  &    0.10  \\ 
  Reasons: social and emotional problems  &    0.18  &    0.15  &    0.21  &    0.22  &    0.28  \\ 
  Reasons: performance and learning problems  &    0.94  &    0.92  &    0.67  &    0.88  &    0.78  \\ 
  Reasons: problems with teachers or school  &    0.05  &    0.01  &    0.03  &    0.02  &    0.04  \\ 
  Reasons: not specified  &    0.00  &    0.01  &    0.17  &    0.01  &    0.02  \\ 
  Referred by: Caseworker  &    0.02  &    0.04  &    0.01  &    0.01  &    0.05  \\ 
  Referred by: Other  &    0.01  &    0.02  &    0.17  &    0.03  &    0.07  \\ 
  Referred by: Parents  &    0.04  &    0.05  &    0.11  &    0.02  &    0.06  \\ 
  Referred by: Parents and teacher  &    0.64  &    0.71  &    0.49  &    0.61  &    0.53  \\ 
  Referred by: Teacher  &    0.28  &    0.18  &    0.22  &    0.33  &    0.29  \\ 
  Total number of SPS visits  &   10.27 (7.72) &    9.09 (6.15) &    5.36 (4.61) &   13.58 (9.25) &   19.62 (14.79) \\ 
  Regional office: Ro  &    0.04  &    0.15  &    0.14  &    0.15  &    0.14  \\ 
  Regional office: Go  &    0.02  &    0.13  &    0.10  &    0.12  &    0.12  \\ 
  Regional office: Wi  &    0.12  &    0.18  &    0.15  &    0.25  &    0.13  \\ 
  Regional office: Wa  &    0.17  &    0.12  &    0.10  &    0.07  &    0.19  \\ 
  Regional office: Ra  &    0.38  &    0.07  &    0.15  &    0.06  &    0.20  \\ 
  Regional office: Sa  &    0.20  &    0.18  &    0.18  &    0.18  &    0.15  \\ 
  Regional office: Re  &    0.06  &    0.17  &    0.17  &    0.18  &    0.08  \\ 
  
  \addlinespace[1em]
  \multicolumn{5}{l}{\textbf{B: Sample attrition}}  \\
  In a SW8 cohort  &    0.89  &    0.75  &    0.64  &    0.69  &    0.82  \\ 
  In AHV data  &    0.58  &    0.70  &    0.70  &    0.81  &    0.64  \\ 
  In both SW8 and AHV data  &    0.47  &    0.46  &    0.36  &    0.53  &    0.47  \\ 
 
  \addlinespace[1em]
  \multicolumn{5}{l}{\textbf{C: Outcomes}}  \\
  SW8 Test taken (in SW8 cohort)&    0.86  &    0.82  &    0.71  &    0.80  &    0.41  \\ 
  SW8 Math and German (std.)    &   -0.34 (0.83) &    0.13 (0.85) &    0.41 (0.96) &   -1.20 (0.89) &   -0.30 (1.09) \\ 
  %Chose VET                     &    0.54 (0.50) &    0.61 (0.49) &    0.45 (0.50) &    0.65 (0.48) &    0.36 (0.48) \\ 
  %Chose no further education    &    0.44 (0.50) &    0.35 (0.48) &    0.45 (0.50) &    0.35 (0.48) &    0.62 (0.48) \\ 
  Used disability insurance     &    0.04  &    0.03  &    0.06  &    0.11  &    0.38  \\ 
  Used unemployment insurance   &    0.19  &    0.19  &    0.24  &    0.39  &    0.25  \\ 
  Income (std.)                 &    0.12 (0.97) &    0.15 (0.96) &   -0.05 (1.02) &   -0.15 (0.99) &   -0.56 (0.94) \\ 

\bottomrule
\end{tabular}
\caption{Summary statistics per treatment group} 
\floatfoot{Summary statistics for the population of students referred to the SPS in the Canton of St.\ Gallen. The names of Regional offices are abbreviated for confidentiality purposes. The sample is composed of SN students from the Canton of St.\ Gallen having visited the SPS between 1998 and 2010 and being born between 1982 and 2003. Mean per treatment groups are reported, and standard deviations are reported in parentheses for continuous variables. \emph{Source: SPS}}
\label{table:summary_stats_treatment}
\end{table}

==> Tables/CATE.NONE.ISF.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, Aug 18, 2020 - 5:30:56 PM
\begin{table}[!htbp] \centering 
  \caption{GATEs: KK-ISF} 
  \label{} 
\footnotesize 
\begin{tabular}{@{\extracolsep{-7.5pt}}lcccccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{12}{c}{Trimmed (abs. values)} \\ 
\cline{2-13} 
 & \multicolumn{3}{c}{Probability of taking the SW8 test} & \multicolumn{3}{c}{SW8 test results} & \multicolumn{3}{c}{Work income} & \multicolumn{3}{c}{Probability of using DI} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12)\\ 
\hline \\[-1.8ex] 
 Constant & $-$0.03$^{***}$ & $-$0.01 & $-$0.01 & $-$0.34$^{***}$ & $-$0.36$^{***}$ & $-$0.35$^{***}$ & 0.11$^{***}$ & 0.07 & 0.13$^{***}$ & $-$0.02 & $-$0.03 & $-$0.02 \\ 
  & (0.01) & (0.01) & (0.01) & (0.01) & (0.02) & (0.01) & (0.03) & (0.05) & (0.04) & (0.04) & (0.06) & (0.04) \\ 
  & & & & & & & & & & & & \\ 
 Female &  & $-$0.05$^{**}$ &  &  & 0.05$^{*}$ &  &  & 0.09 &  &  & 0.01 &  \\ 
  &  & (0.02) &  &  & (0.03) &  &  & (0.07) &  &  & (0.08) &  \\ 
  & & & & & & & & & & & & \\ 
 Non-native &  &  & $-$0.15$^{***}$ &  &  & 0.15$^{**}$ &  &  & $-$0.28$^{***}$ &  &  & $-$0.03 \\ 
  &  &  & (0.05) &  &  & (0.07) &  &  & (0.10) &  &  & (0.19) \\ 
  & & & & & & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 9,960 & 9,960 & 9,960 & 7,900 & 7,900 & 7,900 & 10,113 & 10,113 & 10,113 & 10,152 & 10,152 & 10,152 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{12}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Tables/CATE.NONE.KK.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, Aug 18, 2020 - 5:31:14 PM
\begin{table}[!htbp] \centering 
  \caption{GATEs: KK-ISF} 
  \label{} 
\footnotesize 
\begin{tabular}{@{\extracolsep{-7.5pt}}lcccccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{12}{c}{Trimmed (abs. values)} \\ 
\cline{2-13} 
 & \multicolumn{3}{c}{Probability of taking the SW8 test} & \multicolumn{3}{c}{SW8 test results} & \multicolumn{3}{c}{Work income} & \multicolumn{3}{c}{Probability of using DI} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12)\\ 
\hline \\[-1.8ex] 
 Constant & $-$0.03$^{**}$ & $-$0.03$^{*}$ & $-$0.03$^{**}$ & $-$0.85$^{***}$ & $-$0.83$^{***}$ & $-$0.88$^{***}$ & $-$0.07$^{**}$ & $-$0.02 & $-$0.09$^{***}$ & 0.01 & $-$0.003 & 0.01 \\ 
  & (0.01) & (0.02) & (0.01) & (0.01) & (0.02) & (0.02) & (0.03) & (0.04) & (0.03) & (0.04) & (0.05) & (0.04) \\ 
  & & & & & & & & & & & & \\ 
 Female &  & $-$0.01 &  &  & $-$0.03 &  &  & $-$0.11$^{*}$ &  &  & 0.03 &  \\ 
  &  & (0.03) &  &  & (0.03) &  &  & (0.06) &  &  & (0.09) &  \\ 
  & & & & & & & & & & & & \\ 
 Non-native &  &  & $-$0.03 &  &  & 0.29$^{***}$ &  &  & 0.38$^{***}$ &  &  & $-$0.03 \\ 
  &  &  & (0.05) &  &  & (0.05) &  &  & (0.09) &  &  & (0.23) \\ 
  & & & & & & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 9,963 & 9,963 & 9,963 & 7,899 & 7,899 & 7,899 & 10,115 & 10,115 & 10,115 & 10,154 & 10,154 & 10,154 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{12}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Tables/CATE.NONE.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, Aug 18, 2020 - 5:26:35 PM
\begin{table}[!htbp] \centering 
  \caption{GATEs: KK-ISF} 
  \label{} 
\footnotesize 
\begin{tabular}{@{\extracolsep{-7.5pt}}lcccccccccccccccccccccccccccccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{36}{c}{Trimmed (abs. values)} \\ 
\cline{2-37} 
 & \multicolumn{3}{c}{Probability of taking the SW8 test} & \multicolumn{3}{c}{SW8 test results} & \multicolumn{3}{c}{Work income} & \multicolumn{3}{c}{Probability of using DI} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) & (14) & (15) & (16) & (17) & (18) & (19) & (20) & (21) & (22) & (23) & (24) & (25) & (26) & (27) & (28) & (29) & (30) & (31) & (32) & (33) & (34) & (35) & (36)\\ 
\hline \\[-1.8ex] 
 Constant & $-$0.03$^{***}$ & $-$0.01 & $-$0.01 & $-$0.03$^{**}$ & $-$0.03$^{*}$ & $-$0.03$^{**}$ & $-$0.30$^{***}$ & $-$0.27$^{***}$ & $-$0.30$^{***}$ & $-$0.34$^{***}$ & $-$0.36$^{***}$ & $-$0.35$^{***}$ & $-$0.85$^{***}$ & $-$0.83$^{***}$ & $-$0.88$^{***}$ & $-$0.40$^{***}$ & $-$0.42$^{***}$ & $-$0.43$^{***}$ & 0.11$^{***}$ & 0.07 & 0.13$^{***}$ & $-$0.07$^{**}$ & $-$0.02 & $-$0.09$^{***}$ & $-$0.34$^{***}$ & $-$0.36$^{***}$ & $-$0.36$^{***}$ & $-$0.02 & $-$0.03 & $-$0.02 & 0.01 & $-$0.003 & 0.01 & 0.16$^{***}$ & 0.15$^{***}$ & 0.16$^{***}$ \\ 
  & (0.01) & (0.01) & (0.01) & (0.01) & (0.02) & (0.01) & (0.02) & (0.02) & (0.02) & (0.01) & (0.02) & (0.01) & (0.01) & (0.02) & (0.02) & (0.01) & (0.02) & (0.01) & (0.03) & (0.05) & (0.04) & (0.03) & (0.04) & (0.03) & (0.02) & (0.03) & (0.02) & (0.04) & (0.06) & (0.04) & (0.04) & (0.05) & (0.04) & (0.04) & (0.05) & (0.04) \\ 
  & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\ 
 Female &  & $-$0.05$^{**}$ &  &  & $-$0.01 &  &  & $-$0.06$^{*}$ &  &  & 0.05$^{*}$ &  &  & $-$0.03 &  &  & 0.05$^{**}$ &  &  & 0.09 &  &  & $-$0.11$^{*}$ &  &  & 0.04 &  &  & 0.01 &  &  & 0.03 &  &  & 0.02 &  \\ 
  &  & (0.02) &  &  & (0.03) &  &  & (0.03) &  &  & (0.03) &  &  & (0.03) &  &  & (0.02) &  &  & (0.07) &  &  & (0.06) &  &  & (0.05) &  &  & (0.08) &  &  & (0.09) &  &  & (0.08) &  \\ 
  & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\ 
 Non-native &  &  & $-$0.15$^{***}$ &  &  & $-$0.03 &  &  & 0.05 &  &  & 0.15$^{**}$ &  &  & 0.29$^{***}$ &  &  & 0.29$^{***}$ &  &  & $-$0.28$^{***}$ &  &  & 0.38$^{***}$ &  &  & 0.26$^{***}$ &  &  & $-$0.03 &  &  & $-$0.03 &  &  & $-$0.04 \\ 
  &  &  & (0.05) &  &  & (0.05) &  &  & (0.05) &  &  & (0.07) &  &  & (0.05) &  &  & (0.03) &  &  & (0.10) &  &  & (0.09) &  &  & (0.09) &  &  & (0.19) &  &  & (0.23) &  &  & (0.17) \\ 
  & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 9,960 & 9,960 & 9,960 & 9,963 & 9,963 & 9,963 & 9,966 & 9,966 & 9,966 & 7,900 & 7,900 & 7,900 & 7,899 & 7,899 & 7,899 & 7,902 & 7,902 & 7,902 & 10,113 & 10,113 & 10,113 & 10,115 & 10,115 & 10,115 & 10,120 & 10,120 & 10,120 & 10,152 & 10,152 & 10,152 & 10,154 & 10,154 & 10,154 & 10,159 & 10,159 & 10,159 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{36}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Tables/CATE.dict.interest.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, Aug 18, 2020 - 5:49:44 PM
\begin{table}[!htbp] \centering 
  \caption{GATEs: KK-ISF} 
  \label{} 
\tiny 
\begin{tabular}{@{\extracolsep{-7.5pt}}lcccccccccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{16}{c}{Trimmed (abs. values)} \\ 
\cline{2-17} 
 & \multicolumn{4}{c}{Probability of taking the SW8 test} & \multicolumn{4}{c}{SW8 test results} & \multicolumn{4}{c}{Work income} & \multicolumn{4}{c}{Probability of using DI} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) & (14) & (15) & (16)\\ 
\hline \\[-1.8ex] 
 Constant & $-$0.01 & 0.004 & $-$0.004 & $-$0.003 & $-$0.51$^{***}$ & $-$0.54$^{***}$ & $-$0.51$^{***}$ & $-$0.51$^{***}$ & $-$0.18$^{***}$ & $-$0.18$^{***}$ & $-$0.18$^{***}$ & $-$0.18$^{***}$ & 0.03 & 0.04 & 0.03 & 0.03 \\ 
  & (0.01) & (0.02) & (0.01) & (0.01) & (0.02) & (0.02) & (0.02) & (0.02) & (0.04) & (0.04) & (0.04) & (0.04) & (0.04) & (0.05) & (0.04) & (0.04) \\ 
  & & & & & & & & & & & & & & & & \\ 
 Konzentrationsstoerung & 0.14$^{***}$ &  &  &  & 0.04 &  &  &  & 0.04 &  &  &  & 0.0002 &  &  &  \\ 
  & (0.02) &  &  &  & (0.08) &  &  &  & (0.05) &  &  &  & (0.18) &  &  &  \\ 
  & & & & & & & & & & & & & & & & \\ 
 Leistungsstoerung &  & $-$0.03$^{*}$ &  &  &  & 0.11$^{***}$ &  &  &  & 0.003 &  &  &  & $-$0.02 &  &  \\ 
  &  & (0.02) &  &  &  & (0.03) &  &  &  & (0.07) &  &  &  & (0.10) &  &  \\ 
  & & & & & & & & & & & & & & & & \\ 
 Leistungsstoerung &  &  & 0.03 &  &  &  & $-$0.10$^{***}$ &  &  &  & 0.17 &  &  &  & 0.06 &  \\ 
  &  &  & (0.07) &  &  &  & (0.03) &  &  &  & (0.13) &  &  &  & (0.17) &  \\ 
  & & & & & & & & & & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 9,961 & 9,961 & 9,961 & 9,961 & 7,898 & 7,898 & 7,898 & 7,898 & 10,115 & 10,115 & 10,115 & 10,115 & 10,154 & 10,154 & 10,154 & 10,154 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{16}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Tables/CATE.interest.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, Aug 18, 2020 - 5:47:28 PM
\begin{table}[!htbp] \centering 
  \caption{GATEs: KK-ISF} 
  \label{} 
\footnotesize 
\begin{tabular}{@{\extracolsep{-7.5pt}}lcccccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{12}{c}{Trimmed (abs. values)} \\ 
\cline{2-13} 
 & \multicolumn{4}{c}{Probability of taking the SW8 test} & \multicolumn{4}{c}{SW8 test results} & \multicolumn{4}{c}{Work income} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12)\\ 
\hline \\[-1.8ex] 
 Constant & $-$0.003 & $-$0.02 & $-$0.02 & $-$0.51$^{***}$ & $-$0.47$^{***}$ & $-$0.53$^{***}$ & $-$0.18$^{***}$ & $-$0.10$^{***}$ & $-$0.22$^{***}$ & 0.03 & 0.02 & 0.03 \\ 
  & (0.01) & (0.02) & (0.01) & (0.01) & (0.02) & (0.02) & (0.02) & (0.02) & (0.04) & (0.04) & (0.04) & (0.04) \\ 
  & & & & & & & & & & & & \\ 
 Female &  & 0.04 &  &  & $-$0.09 &  &  & $-$0.20 &  &  & 0.02 &  \\ 
  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  & & & & & & & & & & & & \\ 
 Non-native &  &  & 0.11 &  &  & 0.14 &  &  & 0.66 &  &  & 0.004 \\ 
  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
  & & & & & & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 9,961 & 9,961 & 9,961 & 7,898 & 7,898 & 7,898 & 10,115 & 10,115 & 10,115 & 10,154 & 10,154 & 10,154 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{12}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Tables/GATE.dict.KKISF.SW8.UBD.nontrimmed.FULL.weight.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Wed, Nov 04, 2020 - 2:11:38 PM
\begin{table}[!htbp] \centering 
  \caption{GATEs on segregation vs inclusion} 
  \label{table:GATE.dict} 
\tiny 
\begin{tabular}{@{\extracolsep{3pt}}lcccccccccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{16}{c}{Semi-segregation vs. inclusion} \\ 
\cline{2-17} 
 & \multicolumn{8}{c}{SW8 test results} & \multicolumn{8}{c}{Probability of being unemployed} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) & (14) & (15) & (16)\\ 
\hline \\[-1.8ex] 
 Constant & $-$0.586$^{***}$ & $-$0.655$^{***}$ & $-$0.787$^{***}$ & $-$0.608$^{***}$ & $-$0.582$^{***}$ & $-$0.644$^{***}$ & $-$0.654$^{***}$ & $-$0.968$^{**}$ & 0.204$^{***}$ & 0.155$^{***}$ & 0.086$^{*}$ & 0.084 & 0.139$^{***}$ & 0.123$^{***}$ & 0.032 & 0.090 \\ 
  & (0.126) & (0.168) & (0.184) & (0.186) & (0.121) & (0.097) & (0.191) & (0.412) & (0.049) & (0.047) & (0.047) & (0.060) & (0.041) & (0.038) & (0.053) & (0.058) \\ 
  & & & & & & & & & & & & & & & & \\ 
 Conflict with teacher & $-$0.549 &  &  &  &  &  &  & $-$0.290 & $-$1.405$^{**}$ &  &  &  &  &  &  & $-$1.468$^{**}$ \\ 
  & (2.430) &  &  &  &  &  &  & (2.593) & (0.692) &  &  &  &  &  &  & (0.668) \\ 
  & & & & & & & & & & & & & & & & \\ 
 ADHD &  & 0.636 &  &  &  &  &  & 0.371 &  & $-$0.453 &  &  &  &  &  & $-$0.584 \\ 
  &  & (2.668) &  &  &  &  &  & (3.110) &  & (0.597) &  &  &  &  &  & (0.706) \\ 
  & & & & & & & & & & & & & & & & \\ 
 Performance issues &  &  & 2.228 &  &  &  &  & 2.887 &  &  & 0.555 &  &  &  &  & 0.757 \\ 
  &  &  & (2.214) &  &  &  &  & (2.551) &  &  & (0.516) &  &  &  &  & (0.509) \\ 
  & & & & & & & & & & & & & & & & \\ 
 Learning difficulties &  &  &  & $-$0.121 &  &  &  & $-$1.479 &  &  &  & 0.720 &  &  &  & $-$0.229 \\ 
  &  &  &  & (2.758) &  &  &  & (4.152) &  &  &  & (1.005) &  &  &  & (1.229) \\ 
  & & & & & & & & & & & & & & & & \\ 
 Able to attend school &  &  &  &  & $-$0.622 &  &  & $-$0.093 &  &  &  &  & $-$0.205 &  &  & $-$0.783 \\ 
  &  &  &  &  & (2.181) &  &  & (2.777) &  &  &  &  & (0.439) &  &  & (0.512) \\ 
  & & & & & & & & & & & & & & & & \\ 
 Behavioral and social problems &  &  &  &  &  & 0.462 &  & 1.365 &  &  &  &  &  & 0.070 &  & 0.570 \\ 
  &  &  &  &  &  & (1.436) &  & (1.702) &  &  &  &  &  & (0.411) &  & (0.393) \\ 
  & & & & & & & & & & & & & & & & \\ 
 Language and speech issues &  &  &  &  &  &  & 0.608 & 2.156 &  &  &  &  &  &  & 1.544$^{**}$ & 1.904$^{**}$ \\ 
  &  &  &  &  &  &  & (2.710) & (3.557) &  &  &  &  &  &  & (0.659) & (0.827) \\ 
  & & & & & & & & & & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 10,382 & 10,382 & 10,382 & 10,382 & 10,382 & 10,382 & 10,382 & 10,382 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 \\ 
F Statistic & 0.026 & 0.028 & 0.679 & 0.001 & 0.029 & 0.048 & 0.035 & 0.170 & 1.567 & 0.130 & 0.409 & 0.300 & 0.031 & 0.006 & 1.732 & 0.653 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{16}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Tables/GATE.dict.KKISF.WAGE.DID.nontrimmed.FULL.weight.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Wed, Nov 04, 2020 - 2:11:45 PM
\begin{table}[!htbp] \centering 
  \caption{GATEs on segregation vs inclusion} 
  \label{table:GATE.dict} 
\tiny 
\begin{tabular}{@{\extracolsep{3pt}}lcccccccccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{16}{c}{Semi-segregation vs. inclusion} \\ 
\cline{2-17} 
 & \multicolumn{8}{c}{Probability of using DI} & \multicolumn{8}{c}{Work income (month)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) & (14) & (15) & (16)\\ 
\hline \\[-1.8ex] 
 Constant & 0.031 & 0.023 & 0.007 & $-$0.019 & 0.028 & 0.028 & $-$0.010 & 0.037 & $-$0.201$^{**}$ & $-$0.098 & $-$0.137 & $-$0.149 & $-$0.288$^{***}$ & $-$0.228$^{***}$ & $-$0.306$^{***}$ & $-$0.141 \\ 
  & (0.023) & (0.026) & (0.032) & (0.033) & (0.028) & (0.022) & (0.044) & (0.046) & (0.082) & (0.075) & (0.086) & (0.093) & (0.086) & (0.076) & (0.101) & (0.126) \\ 
  & & & & & & & & & & & & & & & & \\ 
 Conflict with teacher & $-$0.341 &  &  &  &  &  &  & $-$0.231 & $-$0.354 &  &  &  &  &  &  & $-$0.034 \\ 
  & (0.357) &  &  &  &  &  &  & (0.316) & (1.070) &  &  &  &  &  &  & (1.066) \\ 
  & & & & & & & & & & & & & & & & \\ 
 ADHD &  & $-$0.185 &  &  &  &  &  & $-$0.297 &  & $-$2.020$^{*}$ &  &  &  &  &  & $-$1.867 \\ 
  &  & (0.246) &  &  &  &  &  & (0.255) &  & (1.086) &  &  &  &  &  & (1.143) \\ 
  & & & & & & & & & & & & & & & & \\ 
 Performance issues &  &  & 0.060 &  &  &  &  & 0.035 &  &  & $-$1.117 &  &  &  &  & $-$0.752 \\ 
  &  &  & (0.209) &  &  &  &  & (0.232) &  &  & (0.780) &  &  &  &  & (0.768) \\ 
  & & & & & & & & & & & & & & & & \\ 
 Learning difficulties &  &  &  & 0.513 &  &  &  & 0.459 &  &  &  & $-$1.172 &  &  &  & $-$1.886 \\ 
  &  &  &  & (0.380) &  &  &  & (0.415) &  &  &  & (1.260) &  &  &  & (1.640) \\ 
  & & & & & & & & & & & & & & & & \\ 
 Able to attend school &  &  &  &  & $-$0.299 &  &  & $-$0.563$^{**}$ &  &  &  &  & 1.258 &  &  & 0.987 \\ 
  &  &  &  &  & (0.230) &  &  & (0.261) &  &  &  &  & (0.920) &  &  & (1.022) \\ 
  & & & & & & & & & & & & & & & & \\ 
 Behavioral and social problems &  &  &  &  &  & $-$0.272 &  & $-$0.197 &  &  &  &  &  & 0.131 &  & 0.401 \\ 
  &  &  &  &  &  & (0.242) &  & (0.202) &  &  &  &  &  & (0.802) &  & (0.780) \\ 
  & & & & & & & & & & & & & & & & \\ 
 Language and speech issues &  &  &  &  &  &  & 0.357 & 0.276 &  &  &  &  &  &  & 1.394 & 2.105 \\ 
  &  &  &  &  &  &  & (0.462) & (0.516) &  &  &  &  &  &  & (1.229) & (1.555) \\ 
  & & & & & & & & & & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 \\ 
F Statistic & 0.199 & 0.047 & 0.010 & 0.326 & 0.143 & 0.194 & 0.199 & 0.153 & 0.026 & 0.676 & 0.432 & 0.207 & 0.308 & 0.005 & 0.368 & 0.295 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{16}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Tables/GATE.main.KKISF.nontrimmed.FULL.weight.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Nov 05, 2020 - 4:12:58 PM
\begin{table}[!htbp] \centering 
  \caption{GATEs on segregation vs inclusion} 
  \label{table:GATE.FNAO} 
\tiny 
\begin{tabular}{@{\extracolsep{2pt}}lcccccccccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{16}{c}{Semi-segregation vs. inclusion} \\ 
\cline{2-17} 
 & \multicolumn{4}{c}{SW8 test results} & \multicolumn{4}{c}{Probability of being unemployed} & \multicolumn{4}{c}{Probability of using DI} & \multicolumn{4}{c}{Work income (month)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) & (14) & (15) & (16)\\ 
\hline \\[-1.8ex] 
 Constant & $-$0.615$^{***}$ & $-$0.547$^{***}$ & $-$0.664$^{***}$ & $-$0.696$^{***}$ & 0.128$^{***}$ & 0.121$^{***}$ & 0.139$^{***}$ & 0.146$^{***}$ & 0.012 & 0.040$^{*}$ & 0.011 & 0.033$^{**}$ & $-$0.220$^{***}$ & $-$0.160$^{**}$ & $-$0.273$^{***}$ & $-$0.223$^{***}$ \\ 
  & (0.050) & (0.063) & (0.054) & (0.053) & (0.030) & (0.034) & (0.032) & (0.031) & (0.021) & (0.023) & (0.022) & (0.016) & (0.060) & (0.074) & (0.062) & (0.063) \\ 
  & & & & & & & & & & & & & & & & \\ 
 Female &  & $-$0.160 &  &  &  & 0.017 &  &  &  & $-$0.072 &  &  &  & $-$0.152 &  &  \\ 
  &  & (0.103) &  &  &  & (0.067) &  &  &  & (0.045) &  &  &  & (0.125) &  &  \\ 
  & & & & & & & & & & & & & & & & \\ 
 Nonnative speaker &  &  & 0.415$^{***}$ &  &  &  & $-$0.192$^{*}$ &  &  &  & 0.011 &  &  &  & 0.863$^{***}$ &  \\ 
  &  &  & (0.154) &  &  &  & (0.108) &  &  &  & (0.060) &  &  &  & (0.252) &  \\ 
  & & & & & & & & & & & & & & & & \\ 
 Social and emotional problems &  &  &  & 0.422$^{***}$ &  &  &  & $-$0.138 &  &  &  & $-$0.160 &  &  &  & 0.019 \\ 
  &  &  &  & (0.150) &  &  &  & (0.115) &  &  &  & (0.116) &  &  &  & (0.190) \\ 
  & & & & & & & & & & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 10,382 & 10,382 & 10,382 & 10,382 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 \\ 
F Statistic &  & 2.470 & 6.982$^{***}$ & 10.897$^{***}$ &  & 0.075 & 2.274 & 2.379 &  & 2.826$^{*}$ & 0.016 & 6.856$^{***}$ &  & 1.548 & 12.022$^{***}$ & 0.012 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{16}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Tables/GATE.set2.KKISF.nontrimmed.FULL.weight.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Wed, Nov 04, 2020 - 1:05:41 PM
\begin{table}[!htbp] \centering 
  \caption{GATEs on segregation vs inclusion} 
  \label{table:GATE.Set2} 
\tiny 
\begin{tabular}{@{\extracolsep{3pt}}lccccccccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{15}{c}{Semi-segregation vs. inclusion} \\ 
\cline{2-16} 
 & \multicolumn{5}{c}{SW8 test results} & \multicolumn{5}{c}{Probability of being unemployed} & \multicolumn{5}{c}{Work income (month)} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) & (14) & (15)\\ 
\hline \\[-1.8ex] 
 Constant & $-$0.611$^{***}$ & $-$0.658$^{***}$ & $-$0.643$^{***}$ & $-$0.613$^{***}$ & $-$0.672$^{***}$ & 0.126$^{***}$ & 0.154$^{***}$ & 0.140$^{***}$ & 0.128$^{***}$ & 0.162$^{***}$ & $-$0.222$^{***}$ & $-$0.232$^{***}$ & $-$0.239$^{***}$ & $-$0.225$^{***}$ & $-$0.251$^{***}$ \\ 
  & (0.051) & (0.051) & (0.052) & (0.051) & (0.053) & (0.031) & (0.029) & (0.031) & (0.031) & (0.029) & (0.060) & (0.058) & (0.061) & (0.060) & (0.058) \\ 
  & & & & & & & & & & & & & & & \\ 
 Gifted & $-$0.698 &  &  &  & $-$0.716 & 0.418 &  &  &  & 0.493 & 0.716 &  &  &  & 0.687 \\ 
  & (0.619) &  &  &  & (0.621) & (0.315) &  &  &  & (0.320) & (0.875) &  &  &  & (0.877) \\ 
  & & & & & & & & & & & & & & & \\ 
 Psychological problems &  & 0.405$^{**}$ &  &  & 0.374$^{*}$ &  & $-$0.407$^{*}$ &  &  & $-$0.379$^{*}$ &  & 0.172 &  &  & 0.109 \\ 
  &  & (0.203) &  &  & (0.207) &  & (0.221) &  &  & (0.226) &  & (0.390) &  &  & (0.398) \\ 
  & & & & & & & & & & & & & & & \\ 
 Individual learning goals &  &  & 0.566$^{**}$ &  & 0.508$^{**}$ &  &  & $-$0.482$^{***}$ &  & $-$0.411$^{**}$ &  &  & 0.702$^{*}$ &  & 0.669$^{*}$ \\ 
  &  &  & (0.228) &  & (0.233) &  &  & (0.186) &  & (0.196) &  &  & (0.370) &  & (0.386) \\ 
  & & & & & & & & & & & & & & & \\ 
 Ind. language courses &  &  &  & $-$0.128 & $-$0.147 &  &  &  & $-$0.054 & 0.001 &  &  &  & 0.424 & 0.357 \\ 
  &  &  &  & (0.278) & (0.278) &  &  &  & (0.259) & (0.259) &  &  &  & (0.506) & (0.509) \\ 
  & & & & & & & & & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 10,382 & 10,382 & 10,382 & 10,382 & 10,382 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 & 18,510 \\ 
F Statistic & 1.158 & 6.095$^{**}$ & 5.794$^{**}$ & 0.134 & 3.042$^{**}$ & 0.485 & 11.028$^{***}$ & 6.450$^{**}$ & 0.037 & 4.086$^{***}$ & 0.372 & 0.510 & 3.563$^{*}$ & 0.592 & 1.143 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{15}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Tables/IV_FULL.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Mon, May 24, 2021 - 5:32:40 PM
\begin{table}[t!] \centering 
  \caption{First stage estimates} 
  \label{table:IV.fs} 
\scriptsize 
\begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
\\[-1.8ex] & \multicolumn{7}{c}{Probability to be assigned to inclusive program} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7)\\ 
\hline \\[-1.8ex] 
 School with inclusion & 0.548$^{***}$ & 0.530$^{***}$ & 0.481$^{***}$ & 0.303$^{***}$ & 0.289$^{***}$ & 0.113$^{***}$ & 0.097$^{***}$ \\ 
  & (0.013) & (0.013) & (0.012) & (0.014) & (0.014) & (0.016) & (0.017) \\ 
  & & & & & & & \\ 
 Female &  & 0.037$^{***}$ & 0.028$^{**}$ & 0.023$^{**}$ & 0.023$^{**}$ & 0.022$^{***}$ & 0.027$^{***}$ \\ 
  &  & (0.012) & (0.012) & (0.010) & (0.010) & (0.009) & (0.009) \\ 
  & & & & & & & \\ 
 Nonnative speaker &  & $-$0.184$^{***}$ & $-$0.187$^{***}$ & $-$0.119$^{***}$ & $-$0.085$^{***}$ & $-$0.059$^{***}$ & $-$0.037$^{***}$ \\ 
  &  & (0.016) & (0.015) & (0.014) & (0.015) & (0.012) & (0.013) \\ 
  & & & & & & & \\ 
 Age at first referral &  & $-$0.018$^{***}$ & $-$0.027$^{***}$ & $-$0.027$^{***}$ & $-$0.027$^{***}$ & $-$0.025$^{***}$ & $-$0.023$^{***}$ \\ 
  &  & (0.003) & (0.003) & (0.002) & (0.002) & (0.002) & (0.002) \\ 
  & & & & & & & \\ 
 IQ &  &  &  &  &  &  & 0.005$^{***}$ \\ 
  &  &  &  &  &  &  & (0.0005) \\ 
  & & & & & & & \\ 
 Share of nonnatives in school &  &  &  &  & $-$0.351$^{***}$ &  &  \\ 
  &  &  &  &  & (0.058) &  &  \\ 
  & & & & & & & \\ 
 Constant & 0.290$^{***}$ & 0.477$^{***}$ & 0.370$^{***}$ & 0.184$^{**}$ & 0.200$^{***}$ & $-$0.125 & $-$0.650$^{***}$ \\ 
  & (0.010) & (0.027) & (0.032) & (0.073) & (0.072) & (0.122) & (0.146) \\ 
  & & & & & & & \\ 
Year FE & No & No & Yes & Yes & Yes & Yes & Yes \\ 
Caseworker & No & No & No & Yes & Yes & No & No \\ 
Regional office & No & No & No & No & Yes & Yes & Yes \\ 
School FE & No & No & No & No & No & Yes & Yes \\ 
First stage F stat & 1826.82 & 1747.82 & 1566.19 & 495.22 & 445.31 & 50.44 & 31.69 \\ 
\textit{N} & 4,189 & 4,189 & 4,189 & 4,061 & 4,061 & 4,189 & 3,359 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Notes:} & \multicolumn{7}{r}{$^{***}$Significant at the 1 percent level.} \\ 
 & \multicolumn{7}{r}{$^{**}$Significant at the 5 percent level.} \\ 
 & \multicolumn{7}{r}{$^{*}$Significant at the 10 percent level.} \\ 
 & \multicolumn{7}{r}{Sample without children assigned to full segregated SE.} \\ 
\end{tabular} 
\end{table} 


==> Tables/IV_ISF_KK.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Sat, Aug 28, 2021 - 3:01:31 PM
\begin{table}[t!] \centering 
  \caption{First stage estimates} 
  \label{table:IV.fs} 
\scriptsize 
\begin{tabular}{@{\extracolsep{4pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
\\[-1.8ex] & \multicolumn{7}{c}{Probability to be assigned to inclusive program} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7)\\ 
\hline \\[-1.8ex] 
 School with inclusion & 0.548$^{***}$ & 0.530$^{***}$ & 0.481$^{***}$ & 0.303$^{***}$ & 0.289$^{***}$ & 0.114$^{***}$ & 0.099$^{***}$ \\ 
  & (0.013) & (0.013) & (0.012) & (0.014) & (0.014) & (0.016) & (0.017) \\ 
  & & & & & & & \\ 
 Female &  & 0.037$^{***}$ & 0.028$^{**}$ & 0.023$^{**}$ & 0.023$^{**}$ & 0.022$^{**}$ & 0.026$^{***}$ \\ 
  &  & (0.012) & (0.012) & (0.010) & (0.010) & (0.009) & (0.009) \\ 
  & & & & & & & \\ 
 Nonnative speaker &  & $-$0.184$^{***}$ & $-$0.187$^{***}$ & $-$0.119$^{***}$ & $-$0.083$^{***}$ & $-$0.061$^{***}$ & $-$0.040$^{***}$ \\ 
  &  & (0.016) & (0.015) & (0.014) & (0.015) & (0.012) & (0.013) \\ 
  & & & & & & & \\ 
 Age at first referral &  & $-$0.018$^{***}$ & $-$0.027$^{***}$ & $-$0.027$^{***}$ & $-$0.027$^{***}$ & $-$0.026$^{***}$ & $-$0.024$^{***}$ \\ 
  &  & (0.003) & (0.003) & (0.002) & (0.002) & (0.002) & (0.002) \\ 
  & & & & & & & \\ 
 IQ &  &  &  &  &  &  & 0.005$^{***}$ \\ 
  &  &  &  &  &  &  & (0.0005) \\ 
  & & & & & & & \\ 
 Share of nonnatives in school &  &  &  &  & $-$0.331$^{***}$ &  &  \\ 
  &  &  &  &  & (0.053) &  &  \\ 
  & & & & & & & \\ 
 Constant & 0.290$^{***}$ & 0.477$^{***}$ & 0.370$^{***}$ & 0.184$^{**}$ & 0.194$^{***}$ & 0.053 & $-$0.442$^{***}$ \\ 
  & (0.010) & (0.027) & (0.032) & (0.073) & (0.072) & (0.043) & (0.065) \\ 
  & & & & & & & \\ 
Year FE & No & No & Yes & Yes & Yes & Yes & Yes \\ 
Caseworker & No & No & No & Yes & Yes & No & No \\ 
Regional office & No & No & No & No & Yes & Yes & Yes \\ 
School FE & No & No & No & No & No & Yes & Yes \\ 
First stage F stat & 1826.82 & 1747.82 & 1566.19 & 495.22 & 444.32 & 51.24 & 32.92 \\ 
\textit{N} & 4,189 & 4,189 & 4,189 & 4,061 & 4,061 & 4,189 & 3,359 \\ 
\hline 
\hline \\[-1.8ex] 
\multicolumn{3}{l}{\textit{Notes: Sample with children in ISF and KK only.}} & \multicolumn{4}{r}{$^{***}$Significant at the 1 percent level.} \\ 
 & \multicolumn{7}{r}{$^{**}$Significant at the 5 percent level.} \\ 
 & \multicolumn{7}{r}{$^{*}$Significant at the 10 percent level.} \\ 
\end{tabular} 
\end{table} 


==> Tables/IV_results.tex <==
\begin{table}[!t]

\caption{\label{tab:}IV results of inclusion \label{table:IV_results}}
\centering
\footnotesize
	\begin{tabular}[t]{llcc}
	\toprule
	\multicolumn{4}{c}{IV Estimates: effect of inclusion} \\
	\cmidrule(l{3pt}r{3pt}){1-4}
	Outcome & LATE & Conf. int. low & Conf. int. high\\
	\midrule
	\addlinespace[1em]
	\multicolumn{4}{l}{\textbf{Only inclusion and semi-segregation}}\\
	\hspace{1em}SW8 test results 					& -0.757 	& -0.538 	& -0.977\\
	\hspace{1em}Probability of using DI 			& -0.002 	& 0.073 	& -0.077\\
	\hspace{1em}Probability of being unemployed 	& 0.153 	& 0.280 	& 0.028\\
	\hspace{1em}Work income (month) 				& -0.145 	& 0.131 	& -0.421\\
	\addlinespace[1em]
	%\multicolumn{4}{l}{\textbf{Full sample without hard segregation}}\\
	%\hspace{1em}SW8 test results & 0.445 & 0.657 & 0.233\\
	%\hspace{1em}Probability of being unemployed & -0.063 & 0.000 & -0.126\\
	%\hspace{1em}Probability of using DI & -0.361 & -0.258 & -0.464\\
	%\hspace{1em}Probability of being unemployed & -0.361 & -0.258 & -0.464\\
	%\hspace{1em}Probability of using DI & -0.063 & 0.000 & -0.126\\
	%\hspace{1em}Work income (month) & 0.483 & 0.736 & 0.229\\
	\bottomrule
\end{tabular}
\floatfoot{LATE estimates estimated using generalized random forest with honesty. The forest was grown with 10'000 trees. Text covariates were discovered in a hold-out sample. 95\% confidence intervals are given in the table. \emph{Source: SPS, Pensenpool}.}
\end{table}


==> Tables/junk/CATE.interest.5.95.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Aug 14, 2020 - 6:19:54 PM
\begin{table}[!htbp] \centering 
  \caption{GATEs: test scores and income} 
  \label{} 
\footnotesize 
\begin{tabular}{@{\extracolsep{-7.5pt}}lcccccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{12}{c}{Trimmed (abs. values): 5-95} \\ 
\cline{2-13} 
 & \multicolumn{6}{c}{Test score} & \multicolumn{6}{c}{Income} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12)\\ 
\hline \\[-1.8ex] 
 Constant & $-$0.50$^{***}$ & $-$0.50$^{***}$ & $-$0.51$^{***}$ & 0.47$^{***}$ & 0.46$^{***}$ & 0.47$^{***}$ & $-$0.13$^{***}$ & $-$0.08$^{***}$ & $-$0.15$^{***}$ & $-$0.31$^{***}$ & $-$0.37$^{***}$ & $-$0.31$^{***}$ \\ 
  & (0.02) & (0.02) & (0.02) & (0.01) & (0.02) & (0.01) & (0.02) & (0.03) & (0.02) & (0.02) & (0.03) & (0.02) \\ 
  & & & & & & & & & & & & \\ 
 female &  & $-$0.01 &  &  & 0.02 &  &  & $-$0.14$^{***}$ &  &  & 0.14$^{***}$ &  \\ 
  &  & (0.04) &  &  & (0.03) &  &  & (0.04) &  &  & (0.04) &  \\ 
  & & & & & & & & & & & & \\ 
 nonnative &  &  & 0.09 &  &  & $-$0.001 &  &  & 0.20$^{**}$ &  &  & 0.08 \\ 
  &  &  & (0.06) &  &  & (0.05) &  &  & (0.09) &  &  & (0.08) \\ 
  & & & & & & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 7,840 & 7,840 & 7,840 & 7,866 & 7,866 & 7,866 & 10,022 & 10,022 & 10,022 & 10,035 & 10,035 & 10,035 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{12}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Tables/junk/CATE.interest.pure.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Aug 14, 2020 - 6:31:50 PM
\begin{table}[!htbp] \centering 
  \caption{GATEs: test scores and income} 
  \label{} 
\footnotesize 
\begin{tabular}{@{\extracolsep{-7.5pt}}lcccccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{12}{c}{No trimming} \\ 
\cline{2-13} 
 & \multicolumn{6}{c}{Test score} & \multicolumn{6}{c}{Income} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12)\\ 
\hline \\[-1.8ex] 
 Constant & $-$0.61$^{***}$ & $-$0.58$^{***}$ & $-$0.64$^{***}$ & 0.57$^{***}$ & 0.51$^{***}$ & 0.58$^{***}$ & $-$0.03 & 0.03 & $-$0.07 & $-$0.32$^{***}$ & $-$0.40$^{***}$ & $-$0.32$^{***}$ \\ 
  & (0.08) & (0.10) & (0.09) & (0.07) & (0.08) & (0.08) & (0.10) & (0.09) & (0.11) & (0.09) & (0.07) & (0.09) \\ 
  & & & & & & & & & & & & \\ 
 female &  & $-$0.06 &  &  & 0.15 &  &  & $-$0.14 &  &  & 0.18 &  \\ 
  &  & (0.18) &  &  & (0.15) &  &  & (0.23) &  &  & (0.20) &  \\ 
  & & & & & & & & & & & & \\ 
 nonnative &  &  & 0.25$^{**}$ &  &  & $-$0.14 &  &  & 0.63$^{**}$ &  &  & $-$0.07 \\ 
  &  &  & (0.12) &  &  & (0.10) &  &  & (0.26) &  &  & (0.21) \\ 
  & & & & & & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 7,905 & 7,905 & 7,905 & 7,905 & 7,905 & 7,905 & 10,131 & 10,131 & 10,131 & 10,131 & 10,131 & 10,131 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{12}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Tables/junk/CATE.interest.quant.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Aug 14, 2020 - 6:24:00 PM
\begin{table}[!htbp] \centering 
  \caption{GATEs: test scores and income} 
  \label{} 
\footnotesize 
\begin{tabular}{@{\extracolsep{-7.5pt}}lcccccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{12}{c}{Trimmed (quantiles 0.01-0.09)} \\ 
\cline{2-13} 
 & \multicolumn{6}{c}{Test score} & \multicolumn{6}{c}{Income} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12)\\ 
\hline \\[-1.8ex] 
 Constant & $-$0.61$^{***}$ & $-$0.59$^{***}$ & $-$0.64$^{***}$ & 0.57$^{***}$ & 0.51$^{***}$ & 0.59$^{***}$ & $-$0.02 & 0.03 & $-$0.07 & $-$0.32$^{***}$ & $-$0.39$^{***}$ & $-$0.32$^{***}$ \\ 
  & (0.08) & (0.10) & (0.09) & (0.07) & (0.08) & (0.08) & (0.10) & (0.09) & (0.11) & (0.09) & (0.07) & (0.09) \\ 
  & & & & & & & & & & & & \\ 
 female &  & $-$0.06 &  &  & 0.14 &  &  & $-$0.14 &  &  & 0.18 &  \\ 
  &  & (0.18) &  &  & (0.15) &  &  & (0.24) &  &  & (0.20) &  \\ 
  & & & & & & & & & & & & \\ 
 nonnative &  &  & 0.25$^{**}$ &  &  & $-$0.14 &  &  & 0.69$^{**}$ &  &  & $-$0.08 \\ 
  &  &  & (0.12) &  &  & (0.10) &  &  & (0.28) &  &  & (0.22) \\ 
  & & & & & & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 7,846 & 7,846 & 7,846 & 7,799 & 7,799 & 7,799 & 9,946 & 9,946 & 9,946 & 9,941 & 9,941 & 9,941 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{12}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Tables/junk/CATE.interest.weight.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Aug 14, 2020 - 6:21:26 PM
\begin{table}[!htbp] \centering 
  \caption{GATEs: test scores and income} 
  \label{} 
\footnotesize 
\begin{tabular}{@{\extracolsep{-7.5pt}}lcccccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{12}{c}{Trimmed (abs. values): 5-95} \\ 
\cline{2-13} 
 & \multicolumn{6}{c}{Test score} & \multicolumn{6}{c}{Income} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12)\\ 
\hline \\[-1.8ex] 
 Constant & $-$0.49$^{***}$ & $-$0.49$^{***}$ & $-$0.49$^{***}$ & 0.46$^{***}$ & 0.46$^{***}$ & 0.46$^{***}$ & $-$0.11$^{***}$ & $-$0.09$^{***}$ & $-$0.11$^{***}$ & $-$0.29$^{***}$ & $-$0.31$^{***}$ & $-$0.29$^{***}$ \\ 
  & (0.0003) & (0.0004) & (0.0003) & (0.0004) & (0.001) & (0.0004) & (0.001) & (0.001) & (0.001) & (0.001) & (0.001) & (0.001) \\ 
  & & & & & & & & & & & & \\ 
 female &  & 0.0002 &  &  & 0.001 &  &  & $-$0.03$^{***}$ &  &  & 0.06$^{***}$ &  \\ 
  &  & (0.001) &  &  & (0.001) &  &  & (0.001) &  &  & (0.002) &  \\ 
  & & & & & & & & & & & & \\ 
 nonnative &  &  & 0.001 &  &  & 0.003$^{**}$ &  &  & 0.02$^{***}$ &  &  & 0.03$^{***}$ \\ 
  &  &  & (0.001) &  &  & (0.001) &  &  & (0.002) &  &  & (0.003) \\ 
  & & & & & & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 7,905 & 7,905 & 7,905 & 7,905 & 7,905 & 7,905 & 10,131 & 10,131 & 10,131 & 10,131 & 10,131 & 10,131 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{12}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Tables/junk/GATE.NONE.HAND.tex <==
% Date and time: Fri, Aug 14, 2020 - 11:10:41 AM 
  \begin{table}[!htbp] \centering  
    \caption{GATEs:Probability of taking the SW8 test}  
    \label{}  
 \begin{tabular}{@{\extracolsep{5pt}}lcccccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{12}{c}{Trimmed (abs. values)} \\ 
\cline{2-13} 
 & \multicolumn{9}{c}{KK-ISF} & \multicolumn{3}{c}{SON-KK} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12)\\ 
\hline \\[-1.8ex] 
 Constant & $-$0.511$^{***}$ & $-$0.473$^{***}$ & $-$0.526$^{***}$ & 0.449$^{***}$ & 0.411$^{***}$ & 0.450$^{***}$ & $-$0.177$^{***}$ & $-$0.096$^{*}$ & $-$0.222$^{***}$ & $-$0.273$^{***}$ & $-$0.333$^{***}$ & $-$0.265$^{***}$ \\ 
  & (0.036) & (0.036) & (0.038) & (0.025) & (0.033) & (0.026) & (0.042) & (0.055) & (0.044) & (0.039) & (0.051) & (0.040) \\ 
  & & & & & & & & & & & & \\ 
 female &  & $-$0.087 &  &  & 0.089$^{*}$ &  &  & $-$0.200$^{**}$ &  &  & 0.148$^{*}$ &  \\ 
  &  &  &  &  & (0.050) &  &  & (0.086) &  &  & (0.079) &  \\ 
  & & & & & & & & & & & & \\ 
 nonnative &  &  & 0.139 &  &  & $-$0.003 &  &  & 0.662$^{***}$ &  &  & $-$0.124 \\ 
  &  &  & (0.114) &  &  & (0.079) &  &  & (0.168) &  &  & (0.155) \\ 
  & & & & & & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 7,898 & 7,898 & 7,898 & 7,900 & 7,900 & 7,900 & 10,115 & 10,115 & 10,115 & 10,122 & 10,122 & 10,122 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{12}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular}
  \floatfoot{\textit{Note:}  This table shows OLS coefficients and their heteroscedasticity robust standard errors (in parentheses) of regressions run with the pseudo-outcome defined as described in Section XX. }
  \end{table}  

==> Tables/junk/balance.STM.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Dec 18 12:31:36 2019
\begin{table}
\centering
\begingroup\footnotesize
\begin{tabular}{llccccc}
   Pair & Variable & Method & SD Before & Mean SD after & Max |SD| after & 
                      Min |SD| after \\
 \midrule
ISF KK & Age at first interview & STM & 0.40 & 0.28 & 0.44 & 0.21 \\ 
  ISF KK & Female & STM & 0.05 & 0.06 & 0.10 & 0.01 \\ 
  ISF KK & Foreign & STM & 0.73 & 0.65 & 0.90 & 0.52 \\ 
  ISF KK & Number of interviews & STM & 0.07 & 0.08 & 0.18 & 0.01 \\ 
  ISF KK & RS Gossau & STM & 0.41 & 0.30 & 0.36 & 0.21 \\ 
  ISF KK & RS R-J & STM & 0.90 & 0.74 & 0.81 & 0.67 \\ 
  ISF KK & RS Rebstein & STM & 0.20 & 0.25 & 0.30 & 0.18 \\ 
  ISF KK & RS Rorschach & STM & 0.33 & 0.28 & 0.33 & 0.22 \\ 
  ISF KK & RS Sargans & STM & 0.13 & 0.06 & 0.10 & 0.01 \\ 
  ISF KK & RS SG & STM & 0.63 & 0.45 & 0.57 & 0.39 \\ 
  ISF KK & RS Wattwil & STM & 0.45 & 0.35 & 0.41 & 0.29 \\ 
  ISF KK & RS Wil & STM & 0.15 & 0.07 & 0.12 & 0.01 \\ 
   \midrule
ISF KK & Age at first interview & TIRM & 0.40 & 0.27 & 0.52 & 0.14 \\ 
  ISF KK & Female & TIRM & 0.05 & 0.07 & 0.19 & 0.02 \\ 
  ISF KK & Foreign & TIRM & 0.73 & 0.60 & 0.79 & 0.44 \\ 
  ISF KK & Number of interviews & TIRM & 0.07 & 0.16 & 0.34 & 0.02 \\ 
  ISF KK & RS Gossau & TIRM & 0.41 & 0.14 & 0.28 & 0.01 \\ 
  ISF KK & RS R-J & TIRM & 0.90 & 0.49 & 0.77 & 0.09 \\ 
  ISF KK & RS Rebstein & TIRM & 0.20 & 0.19 & 0.37 & 0.02 \\ 
  ISF KK & RS Rorschach & TIRM & 0.33 & 0.14 & 0.33 & 0.00 \\ 
  ISF KK & RS Sargans & TIRM & 0.13 & 0.17 & 0.27 & 0.05 \\ 
  ISF KK & RS SG & TIRM & 0.63 & 0.40 & 0.56 & 0.04 \\ 
  ISF KK & RS Wattwil & TIRM & 0.45 & 0.28 & 0.43 & 0.12 \\ 
  ISF KK & RS Wil & TIRM & 0.15 & 0.07 & 0.10 & 0.01 \\ 
   \midrule
KK ISF & Age at first interview & STM & 0.40 & 0.15 & 0.23 & 0.00 \\ 
  KK ISF & Female & STM & 0.05 & 0.05 & 0.11 & 0.01 \\ 
  KK ISF & Foreign & STM & 0.73 & 0.46 & 0.65 & 0.31 \\ 
  KK ISF & Number of interviews & STM & 0.07 & 0.06 & 0.14 & 0.02 \\ 
  KK ISF & RS Gossau & STM & 0.41 & 0.23 & 0.34 & 0.12 \\ 
  KK ISF & RS R-J & STM & 0.90 & 0.30 & 0.45 & 0.21 \\ 
  KK ISF & RS Rebstein & STM & 0.20 & 0.08 & 0.16 & 0.04 \\ 
  KK ISF & RS Rorschach & STM & 0.33 & 0.14 & 0.26 & 0.03 \\ 
  KK ISF & RS Sargans & STM & 0.13 & 0.30 & 0.37 & 0.21 \\ 
  KK ISF & RS SG & STM & 0.63 & 0.35 & 0.48 & 0.21 \\ 
  KK ISF & RS Wattwil & STM & 0.45 & 0.22 & 0.37 & 0.12 \\ 
  KK ISF & RS Wil & STM & 0.15 & 0.12 & 0.18 & 0.01 \\ 
   \midrule
KK ISF & Age at first interview & TIRM & 0.40 & 0.16 & 0.24 & 0.07 \\ 
  KK ISF & Female & TIRM & 0.05 & 0.11 & 0.24 & 0.01 \\ 
  KK ISF & Foreign & TIRM & 0.73 & 0.44 & 0.71 & 0.02 \\ 
  KK ISF & Number of interviews & TIRM & 0.07 & 0.09 & 0.22 & 0.02 \\ 
  KK ISF & RS Gossau & TIRM & 0.41 & 0.29 & 0.39 & 0.13 \\ 
  KK ISF & RS R-J & TIRM & 0.90 & 0.33 & 0.52 & 0.18 \\ 
  KK ISF & RS Rebstein & TIRM & 0.20 & 0.08 & 0.26 & 0.02 \\ 
  KK ISF & RS Rorschach & TIRM & 0.33 & 0.20 & 0.30 & 0.12 \\ 
  KK ISF & RS Sargans & TIRM & 0.13 & 0.26 & 0.43 & 0.04 \\ 
  KK ISF & RS SG & TIRM & 0.63 & 0.28 & 0.36 & 0.18 \\ 
  KK ISF & RS Wattwil & TIRM & 0.45 & 0.17 & 0.41 & 0.01 \\ 
  KK ISF & RS Wil & TIRM & 0.15 & 0.08 & 0.18 & 0.01 \\ 
   \bottomrule
\end{tabular}
\endgroup
\caption{STM and TIRM: balancing test} 
\label{tab:stm.balancing}
\end{table}


==> Tables/junk/balance.STM.topic.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Dec 18 12:28:31 2019
\begin{table}
\centering
\begingroup\tiny
\begin{tabular}{llccccc}
  \toprule
  Pair & Variable & Method & SD Before & Mean SD after & Max |SD| after & 
                      Min |SD| after \\
 \midrule
ISF KK & theta.1 & STM & 0.23 & 0.18 & 0.43 & 0.03 \\ 
  ISF KK & theta.10 & STM & 0.55 & 0.38 & 1.01 & 0.10 \\ 
  ISF KK & theta.11 & STM & 0.25 & 0.13 & 0.26 & 0.05 \\ 
  ISF KK & theta.12 & STM & 0.25 & 0.20 & 0.27 & 0.06 \\ 
  ISF KK & theta.13 & STM & 0.47 & 0.33 & 0.82 & 0.12 \\ 
  ISF KK & theta.14 & STM & 0.26 & 0.17 & 0.32 & 0.02 \\ 
  ISF KK & theta.15 & STM & 0.20 & 0.18 & 0.23 & 0.06 \\ 
  ISF KK & theta.16 & STM & 0.18 & 0.02 & 0.04 & 0.01 \\ 
  ISF KK & theta.17 & STM & 0.27 & 0.22 & 0.39 & 0.06 \\ 
  ISF KK & theta.18 & STM & 0.16 & 0.15 & 0.25 & 0.06 \\ 
  ISF KK & theta.19 & STM & 0.67 & 0.52 & 1.04 & 0.07 \\ 
  ISF KK & theta.2 & STM & 0.43 & 0.34 & 0.78 & 0.11 \\ 
  ISF KK & theta.20 & STM & 0.33 & 0.22 & 0.34 & 0.05 \\ 
  ISF KK & theta.3 & STM & 0.25 & 0.20 & 0.38 & 0.02 \\ 
  ISF KK & theta.4 & STM & 0.36 & 0.25 & 0.56 & 0.06 \\ 
  ISF KK & theta.5 & STM & 0.36 & 0.28 & 0.68 & 0.04 \\ 
  ISF KK & theta.6 & STM & 0.34 & 0.25 & 0.51 & 0.02 \\ 
  ISF KK & theta.7 & STM & 0.36 & 0.26 & 0.70 & 0.02 \\ 
  ISF KK & theta.8 & STM & 0.60 & 0.42 & 0.96 & 0.01 \\ 
  ISF KK & theta.9 & STM & 0.39 & 0.25 & 0.92 & 0.00 \\ 
  ISF KK & proj.ISF & TIRM & 1.18 & 0.70 & 1.02 & 0.19 \\ 
  ISF KK & proj.KK & TIRM & 0.96 & 0.49 & 0.68 & 0.33 \\ 
  ISF KK & theta.tt.1 & TIRM & 0.14 & 0.22 & 0.47 & 0.03 \\ 
  ISF KK & theta.tt.10 & TIRM & 0.36 & 0.25 & 0.73 & 0.03 \\ 
  ISF KK & theta.tt.11 & TIRM & 0.30 & 0.19 & 0.32 & 0.03 \\ 
  ISF KK & theta.tt.12 & TIRM & 0.40 & 0.22 & 0.46 & 0.01 \\ 
  ISF KK & theta.tt.13 & TIRM & 0.50 & 0.29 & 0.44 & 0.16 \\ 
  ISF KK & theta.tt.14 & TIRM & 0.20 & 0.15 & 0.42 & 0.00 \\ 
  ISF KK & theta.tt.15 & TIRM & 0.26 & 0.15 & 0.24 & 0.07 \\ 
  ISF KK & theta.tt.16 & TIRM & 0.18 & 0.11 & 0.15 & 0.05 \\ 
  ISF KK & theta.tt.17 & TIRM & 0.34 & 0.25 & 0.46 & 0.07 \\ 
  ISF KK & theta.tt.18 & TIRM & 0.33 & 0.23 & 0.36 & 0.04 \\ 
  ISF KK & theta.tt.19 & TIRM & 0.44 & 0.21 & 0.38 & 0.10 \\ 
  ISF KK & theta.tt.2 & TIRM & 0.29 & 0.17 & 0.41 & 0.00 \\ 
  ISF KK & theta.tt.20 & TIRM & 0.13 & 0.12 & 0.29 & 0.03 \\ 
  ISF KK & theta.tt.3 & TIRM & 0.28 & 0.20 & 0.45 & 0.01 \\ 
  ISF KK & theta.tt.4 & TIRM & 0.24 & 0.18 & 0.44 & 0.03 \\ 
  ISF KK & theta.tt.5 & TIRM & 0.44 & 0.28 & 0.41 & 0.04 \\ 
  ISF KK & theta.tt.6 & TIRM & 0.29 & 0.16 & 0.38 & 0.06 \\ 
  ISF KK & theta.tt.7 & TIRM & 0.27 & 0.11 & 0.26 & 0.02 \\ 
  ISF KK & theta.tt.8 & TIRM & 0.23 & 0.22 & 0.37 & 0.11 \\ 
  ISF KK & theta.tt.9 & TIRM & 0.30 & 0.19 & 0.36 & 0.05 \\ 
  KK ISF & theta.1 & STM & 0.23 & 0.16 & 0.38 & 0.02 \\ 
  KK ISF & theta.10 & STM & 0.55 & 0.37 & 1.13 & 0.01 \\ 
  KK ISF & theta.11 & STM & 0.25 & 0.11 & 0.16 & 0.05 \\ 
  KK ISF & theta.12 & STM & 0.25 & 0.13 & 0.21 & 0.06 \\ 
  KK ISF & theta.13 & STM & 0.47 & 0.31 & 0.93 & 0.04 \\ 
  KK ISF & theta.14 & STM & 0.26 & 0.15 & 0.30 & 0.02 \\ 
  KK ISF & theta.15 & STM & 0.20 & 0.14 & 0.34 & 0.02 \\ 
  KK ISF & theta.16 & STM & 0.18 & 0.17 & 0.26 & 0.07 \\ 
  KK ISF & theta.17 & STM & 0.27 & 0.23 & 0.34 & 0.15 \\ 
  KK ISF & theta.18 & STM & 0.16 & 0.06 & 0.10 & 0.04 \\ 
  KK ISF & theta.19 & STM & 0.67 & 0.37 & 0.83 & 0.07 \\ 
  KK ISF & theta.2 & STM & 0.43 & 0.23 & 0.48 & 0.06 \\ 
  KK ISF & theta.20 & STM & 0.33 & 0.22 & 0.40 & 0.03 \\ 
  KK ISF & theta.3 & STM & 0.25 & 0.18 & 0.38 & 0.03 \\ 
  KK ISF & theta.4 & STM & 0.36 & 0.23 & 0.48 & 0.01 \\ 
  KK ISF & theta.5 & STM & 0.36 & 0.18 & 0.49 & 0.01 \\ 
  KK ISF & theta.6 & STM & 0.34 & 0.19 & 0.43 & 0.03 \\ 
  KK ISF & theta.7 & STM & 0.36 & 0.23 & 0.43 & 0.08 \\ 
  KK ISF & theta.8 & STM & 0.60 & 0.37 & 0.88 & 0.11 \\ 
  KK ISF & theta.9 & STM & 0.39 & 0.24 & 0.56 & 0.02 \\ 
  KK ISF & proj.ISF & TIRM & 1.18 & 0.48 & 0.59 & 0.37 \\ 
  KK ISF & proj.KK & TIRM & 0.96 & 0.67 & 0.86 & 0.52 \\ 
  KK ISF & theta.tt.1 & TIRM & 0.16 & 0.17 & 0.34 & 0.06 \\ 
  KK ISF & theta.tt.10 & TIRM & 0.42 & 0.21 & 0.36 & 0.01 \\ 
  KK ISF & theta.tt.11 & TIRM & 0.35 & 0.22 & 0.29 & 0.10 \\ 
  KK ISF & theta.tt.12 & TIRM & 0.46 & 0.31 & 0.61 & 0.19 \\ 
  KK ISF & theta.tt.13 & TIRM & 0.36 & 0.28 & 0.80 & 0.07 \\ 
  KK ISF & theta.tt.14 & TIRM & 0.31 & 0.15 & 0.31 & 0.03 \\ 
  KK ISF & theta.tt.15 & TIRM & 0.23 & 0.12 & 0.32 & 0.02 \\ 
  KK ISF & theta.tt.16 & TIRM & 0.17 & 0.11 & 0.20 & 0.05 \\ 
  KK ISF & theta.tt.17 & TIRM & 0.16 & 0.10 & 0.29 & 0.00 \\ 
  KK ISF & theta.tt.18 & TIRM & 0.23 & 0.19 & 0.38 & 0.01 \\ 
  KK ISF & theta.tt.19 & TIRM & 0.49 & 0.30 & 0.47 & 0.07 \\ 
  KK ISF & theta.tt.2 & TIRM & 0.35 & 0.19 & 0.46 & 0.02 \\ 
  KK ISF & theta.tt.20 & TIRM & 0.08 & 0.08 & 0.17 & 0.02 \\ 
  KK ISF & theta.tt.3 & TIRM & 0.23 & 0.14 & 0.25 & 0.04 \\ 
  KK ISF & theta.tt.4 & TIRM & 0.35 & 0.26 & 0.42 & 0.04 \\ 
  KK ISF & theta.tt.5 & TIRM & 0.47 & 0.26 & 0.67 & 0.01 \\ 
  KK ISF & theta.tt.6 & TIRM & 0.35 & 0.25 & 0.40 & 0.15 \\ 
  KK ISF & theta.tt.7 & TIRM & 0.24 & 0.13 & 0.29 & 0.03 \\ 
  KK ISF & theta.tt.8 & TIRM & 0.28 & 0.19 & 0.58 & 0.01 \\ 
  KK ISF & theta.tt.9 & TIRM & 0.28 & 0.21 & 0.40 & 0.02 \\ 
   \bottomrule
\end{tabular}
\endgroup
\caption{STM and TIRM: balancing test with topics} 
\label{tab:stm.topic.balancing}
\end{table}


==> Tables/junk/balance.cosine.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Dec 18 10:52:12 2019
\begin{table}
\centering
\begingroup\footnotesize
\begin{tabular}{llcccc}
  \toprule
  Pair & Variable & SD Before & Mean SD after & Max |SD| after & 
                      Min |SD| after \\
 \midrule
ISF - KK & Age at first interview & 0.38 & 0.32 & 0.35 & 0.28 \\ 
  ISF - KK & Female & 0.07 & 0.07 & 0.11 & 0.01 \\ 
  ISF - KK & Foreign & 0.72 & 0.46 & 0.49 & 0.43 \\ 
  ISF - KK & Number of interviews & 0.01 & 0.02 & 0.05 & 0.00 \\ 
  KK - ISF & Age at first interview & 0.38 & 0.15 & 0.22 & 0.05 \\ 
  KK - ISF & Female & 0.07 & 0.03 & 0.09 & 0.00 \\ 
  KK - ISF & Foreign & 0.72 & 0.51 & 0.56 & 0.47 \\ 
  KK - ISF & Number of interviews & 0.01 & 0.02 & 0.07 & 0.00 \\ 
   \bottomrule
\end{tabular}
\endgroup
\caption{Cosine similarity: balancing test} 
\label{tab:cos.balancing}
\end{table}


==> Tables/junk/ols.testtaking.mean.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Mon, Jun 22, 2020 - 3:15:47 PM
\begin{table}[h!] \centering 
  \caption{Mean of test takers according to treatment status} 
  \label{table:ols.treatment.testtaking.mean} 
\footnotesize 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & Probability of taking the test \\ 
\hline \\[-1.8ex] 
 treatmentISF & 0.81$^{***}$ \\ 
  & (0.01) \\ 
  treatmentKK & 0.76$^{***}$ \\ 
  & (0.02) \\ 
  treatmentLEGA & 0.86$^{***}$ \\ 
  & (0.01) \\ 
  treatmentLOGO & 0.71$^{***}$ \\ 
  & (0.01) \\ 
  treatmentDYSK & 0.85$^{***}$ \\ 
  & (0.01) \\ 
  treatmentOTHER & 0.72$^{***}$ \\ 
  & (0.01) \\ 
  treatmentSON & 0.26$^{***}$ \\ 
  & (0.03) \\ 
 \hline \\[-1.8ex] 
Controls & No \\ 
Year FE & No \\ 
Regionalstelle FE & No \\ 
City of St. Gallen & Yes \\ 
Observations & 11'545 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Tables/junk/ols.testtaking.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Feb 20, 2020 - 4:53:27 PM
\begin{table}[h!] \centering 
  \caption{Probability of taking test according to treatment status} 
  \label{table:ols.treatment.testtaking} 
\footnotesize 
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{4}{c}{\textit{Dependent variable:}} \\ 
\cline{2-5} 
\\[-1.8ex] & P. of taking the test & P. of taking the test & P. of taking the test & P. of taking the test \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4)\\ 
\hline \\[-1.8ex] 
 Segr. small classes & $-$0.04$^{**}$ & $-$0.06$^{***}$ & $-$0.08$^{***}$ & $-$0.06$^{***}$ \\ 
  & (0.02) & (0.02) & (0.02) & (0.02) \\ 
  Dyslexia ther. & 0.05$^{***}$ & 0.03$^{**}$ & 0.01 & $-$0.01 \\ 
  & (0.01) & (0.01) & (0.01) & (0.01) \\ 
  Speech ther. & $-$0.09$^{***}$ & $-$0.03$^{**}$ & $-$0.03$^{**}$ & $-$0.07$^{***}$ \\ 
  & (0.01) & (0.01) & (0.01) & (0.02) \\ 
  Dyscalculia ther. & 0.04$^{**}$ & 0.02 & 0.001 & $-$0.02 \\ 
  & (0.02) & (0.02) & (0.02) & (0.02) \\ 
  Other therapies & $-$0.07$^{***}$ & $-$0.04$^{***}$ & $-$0.05$^{***}$ & $-$0.07$^{***}$ \\ 
  & (0.01) & (0.01) & (0.01) & (0.01) \\ 
  Segr. schools & $-$0.47$^{***}$ & $-$0.45$^{***}$ & $-$0.46$^{***}$ & $-$0.40$^{***}$ \\ 
  & (0.03) & (0.03) & (0.03) & (0.04) \\ 
  Constant & 0.81$^{***}$ & 0.49$^{***}$ & 0.39$^{***}$ & 0.23$^{***}$ \\ 
  & (0.01) & (0.02) & (0.03) & (0.03) \\ 
 \hline \\[-1.8ex] 
Controls & No & Yes & Yes & Yes \\ 
Year FE & No & No & No & Yes \\ 
Regionalstelle FE & No & Yes & Yes & Yes \\ 
Observations & 19'430 & 19'430 & 19'430 & 14'001 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{4}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
 & \multicolumn{4}{r}{The reference category is Inclusive special education (ISF)} \\ 
\end{tabular} 
\end{table} 


==> Tables/junk/ols.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Feb 20, 2020 - 4:53:29 PM
\begin{table}[h!] \centering 
  \caption{Unconditional comparison of academic performance} 
  \label{table:ols.treatment} 
\footnotesize 
\begin{tabular}{@{\extracolsep{5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & Composite score & Composite score & Composite score & Math score & Language score \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5)\\ 
\hline \\[-1.8ex] 
 Segr. small classes & $-$0.85$^{***}$ & $-$0.39$^{***}$ & $-$0.38$^{***}$ & $-$0.31$^{***}$ & $-$0.41$^{***}$ \\ 
  & (0.05) & (0.05) & (0.05) & (0.05) & (0.05) \\ 
  Dyslexia ther. & 0.49$^{***}$ & 0.15$^{***}$ & 0.16$^{***}$ & 0.09$^{***}$ & 0.19$^{***}$ \\ 
  & (0.03) & (0.03) & (0.03) & (0.03) & (0.03) \\ 
  Speech ther. & 0.16$^{***}$ & 0.10$^{***}$ & 0.10$^{***}$ & 0.03 & 0.15$^{***}$ \\ 
  & (0.04) & (0.03) & (0.03) & (0.04) & (0.04) \\ 
  Dyscalculia ther. & 0.12$^{***}$ & 0.02 & 0.03 & 0.14$^{***}$ & $-$0.09$^{**}$ \\ 
  & (0.04) & (0.04) & (0.04) & (0.04) & (0.04) \\ 
  Other therapies & 0.47$^{***}$ & 0.18$^{***}$ & 0.18$^{***}$ & 0.18$^{***}$ & 0.14$^{***}$ \\ 
  & (0.03) & (0.02) & (0.02) & (0.03) & (0.02) \\ 
  Segr. schools & $-$0.09 & $-$0.22$^{**}$ & $-$0.22$^{**}$ & $-$0.05 & $-$0.35$^{***}$ \\ 
  & (0.12) & (0.10) & (0.10) & (0.11) & (0.11) \\ 
  Constant & $-$0.32$^{***}$ & $-$3.76$^{***}$ & $-$3.86$^{***}$ & $-$3.49$^{***}$ & $-$3.50$^{***}$ \\ 
  & (0.02) & (0.08) & (0.09) & (0.08) & (0.08) \\ 
 \hline \\[-1.8ex] 
Controls & No & Yes & Yes & Yes & Yes \\ 
Year FE & No & No & Yes & No & No \\ 
Regionalstelle FE & No & Yes & Yes & Yes & Yes \\ 
Observations & 14'840 & 11'036 & 11'036 & 11'036 & 11'036 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
 & \multicolumn{5}{r}{The reference category is Inclusive special education (ISF)} \\ 
\end{tabular} 
\end{table} 


==> Tables/junk/parameters.cosine.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Mon Dec 09 11:29:09 2019
\begin{table}
\centering
\begingroup\footnotesize
\begin{tabular}{ccccccc}
  \toprule
  \multicolumn{4}{c}{Text representation parameters} & \multicolumn{3}{c}{Matching parameters}
                      \\
 Weighting & Stemming & Min. term freq. & Max doc. freq. & 
                      Matching & Exact match. & Caliper  \\
 \midrule
tf & Yes &  50 & 0.90 & Neirest Neighbor & Foreign lang. & 0.10 \\ 
  tf\_idf & No & 100 &  &  &  & 0.30 \\ 
   &  &  &  &  &  & 0.50 \\ 
   \bottomrule
\end{tabular}
\endgroup
\caption{Cosine similarity: parameters} 
\label{tab:cos.parameters}
\end{table}


==> Tables/junk/results.stm.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Dec 18 14:51:27 2019
\begin{table}
\centering
\begingroup\tiny
\begin{tabular}{cccccccccccc}
  \toprule
  & \multicolumn{2}{c}{Text representation} & 
                      \multicolumn{2}{c}{STM parameters} & \multicolumn{2}{c}{Matching parameters}
                      & \multicolumn{4}{c}{Estimates} \\
 Pairwise     & Min. term freq. & Stemming &  STM & 
                      Number of k topics & Matching & Caliper & Post-match &
                      Estimate & Std. error & pvalue \\
 \midrule
ISF - KK & 50.00 & FALSE & STM & 10.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & 0.90 & 0.00 & 0.00 \\ 
  ISF - KK & 50.00 & FALSE & STM & 10.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & 0.80 & 0.00 & 0.00 \\ 
  ISF - KK & 50.00 & FALSE & TIRM & 10.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & 0.93 & 0.01 & 0.00 \\ 
  ISF - KK & 50.00 & FALSE & TIRM & 10.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & 0.60 & 0.01 & 0.00 \\ 
  ISF - KK & 50.00 & TRUE & STM & 10.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & 0.88 & 0.00 & 0.00 \\ 
  ISF - KK & 50.00 & TRUE & STM & 10.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & 0.85 & 0.00 & 0.00 \\ 
  ISF - KK & 50.00 & TRUE & TIRM & 10.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & 0.79 & 0.01 & 0.00 \\ 
  ISF - KK & 50.00 & TRUE & TIRM & 10.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & 0.79 & 0.01 & 0.00 \\ 
  ISF - KK & 100.00 & FALSE & STM & 10.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & 0.87 & 0.00 & 0.00 \\ 
  ISF - KK & 100.00 & FALSE & STM & 10.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & 0.81 & 0.00 & 0.00 \\ 
  ISF - KK & 100.00 & FALSE & TIRM & 10.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & 0.88 & 0.00 & 0.00 \\ 
  ISF - KK & 100.00 & FALSE & TIRM & 10.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & 0.47 & 0.01 & 0.00 \\ 
  ISF - KK & 100.00 & TRUE & STM & 10.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & 0.78 & 0.00 & 0.00 \\ 
  ISF - KK & 100.00 & TRUE & STM & 10.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & 0.74 & 0.00 & 0.00 \\ 
  ISF - KK & 100.00 & TRUE & TIRM & 10.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & 0.77 & 0.01 & 0.00 \\ 
  ISF - KK & 100.00 & TRUE & TIRM & 10.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & 0.62 & 0.01 & 0.00 \\ 
  ISF - KK & 50.00 & FALSE & STM & 20.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & 0.83 & 0.00 & 0.00 \\ 
  ISF - KK & 50.00 & FALSE & STM & 20.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & 0.77 & 0.00 & 0.00 \\ 
  ISF - KK & 50.00 & FALSE & TIRM & 20.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & 0.84 & 0.01 & 0.00 \\ 
  ISF - KK & 50.00 & FALSE & TIRM & 20.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & 0.60 & 0.01 & 0.00 \\ 
  ISF - KK & 50.00 & TRUE & STM & 20.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & 0.86 & 0.00 & 0.00 \\ 
  ISF - KK & 50.00 & TRUE & STM & 20.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & 0.75 & 0.00 & 0.00 \\ 
  ISF - KK & 50.00 & TRUE & TIRM & 20.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & 0.75 & 0.01 & 0.00 \\ 
  ISF - KK & 50.00 & TRUE & TIRM & 20.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & 1.33 & 0.01 & 0.00 \\ 
  ISF - KK & 100.00 & FALSE & STM & 20.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & 0.88 & 0.00 & 0.00 \\ 
  ISF - KK & 100.00 & FALSE & STM & 20.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & 0.57 & 0.00 & 0.00 \\ 
  ISF - KK & 100.00 & FALSE & TIRM & 20.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & 0.73 & 0.00 & 0.00 \\ 
  ISF - KK & 100.00 & FALSE & TIRM & 20.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & 0.25 & 0.01 & 0.00 \\ 
  ISF - KK & 100.00 & TRUE & STM & 20.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & 0.85 & 0.00 & 0.00 \\ 
  ISF - KK & 100.00 & TRUE & STM & 20.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & 0.67 & 0.00 & 0.00 \\ 
  ISF - KK & 100.00 & TRUE & TIRM & 20.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & 0.84 & 0.00 & 0.00 \\ 
  ISF - KK & 100.00 & TRUE & TIRM & 20.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & 0.12 & 0.01 & 0.00 \\ 
  KK - ISF & 50.00 & FALSE & STM & 10.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & -0.83 & 0.00 & 0.00 \\ 
  KK - ISF & 50.00 & FALSE & STM & 10.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & -0.72 & 0.00 & 0.00 \\ 
  KK - ISF & 50.00 & FALSE & TIRM & 10.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & -0.77 & 0.01 & 0.00 \\ 
  KK - ISF & 50.00 & FALSE & TIRM & 10.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & -0.46 & 0.01 & 0.00 \\ 
  KK - ISF & 50.00 & TRUE & STM & 10.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & -0.88 & 0.00 & 0.00 \\ 
  KK - ISF & 50.00 & TRUE & STM & 10.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & -0.70 & 0.00 & 0.00 \\ 
  KK - ISF & 50.00 & TRUE & TIRM & 10.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & -0.75 & 0.01 & 0.00 \\ 
  KK - ISF & 50.00 & TRUE & TIRM & 10.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & -0.58 & 0.01 & 0.00 \\ 
  KK - ISF & 100.00 & FALSE & STM & 10.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & -0.81 & 0.00 & 0.00 \\ 
  KK - ISF & 100.00 & FALSE & STM & 10.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & -0.69 & 0.00 & 0.00 \\ 
  KK - ISF & 100.00 & FALSE & TIRM & 10.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & -0.66 & 0.01 & 0.00 \\ 
  KK - ISF & 100.00 & FALSE & TIRM & 10.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & -0.47 & 0.01 & 0.00 \\ 
  KK - ISF & 100.00 & TRUE & STM & 10.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & -0.82 & 0.00 & 0.00 \\ 
  KK - ISF & 100.00 & TRUE & STM & 10.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & -0.66 & 0.00 & 0.00 \\ 
  KK - ISF & 100.00 & TRUE & TIRM & 10.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & -0.75 & 0.01 & 0.00 \\ 
  KK - ISF & 100.00 & TRUE & TIRM & 10.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & -0.44 & 0.01 & 0.00 \\ 
  KK - ISF & 50.00 & FALSE & STM & 20.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & -0.80 & 0.00 & 0.00 \\ 
  KK - ISF & 50.00 & FALSE & STM & 20.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & -0.55 & 0.00 & 0.00 \\ 
  KK - ISF & 50.00 & FALSE & TIRM & 20.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & -0.74 & 0.01 & 0.00 \\ 
  KK - ISF & 50.00 & FALSE & TIRM & 20.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & -0.46 & 0.01 & 0.00 \\ 
  KK - ISF & 50.00 & TRUE & STM & 20.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & -0.85 & 0.00 & 0.00 \\ 
  KK - ISF & 50.00 & TRUE & STM & 20.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & -0.66 & 0.00 & 0.00 \\ 
  KK - ISF & 50.00 & TRUE & TIRM & 20.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & -0.79 & 0.01 & 0.00 \\ 
  KK - ISF & 50.00 & TRUE & TIRM & 20.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & -0.56 & 0.01 & 0.00 \\ 
  KK - ISF & 100.00 & FALSE & STM & 20.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & -0.80 & 0.00 & 0.00 \\ 
  KK - ISF & 100.00 & FALSE & STM & 20.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & -0.69 & 0.00 & 0.00 \\ 
  KK - ISF & 100.00 & FALSE & TIRM & 20.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & -0.79 & 0.01 & 0.00 \\ 
  KK - ISF & 100.00 & FALSE & TIRM & 20.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & -0.47 & 0.01 & 0.00 \\ 
  KK - ISF & 100.00 & TRUE & STM & 20.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & -0.85 & 0.00 & 0.00 \\ 
  KK - ISF & 100.00 & TRUE & STM & 20.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & -0.69 & 0.00 & 0.00 \\ 
  KK - ISF & 100.00 & TRUE & TIRM & 20.00 & P.score, 1:K & 0.10 & mean & points\_math\_deutsch\_std & -0.77 & 0.01 & 0.00 \\ 
  KK - ISF & 100.00 & TRUE & TIRM & 20.00 & P.score, 1:K & 0.10 & ols & points\_math\_deutsch\_std & -0.46 & 0.01 & 0.00 \\ 
   \bottomrule
\end{tabular}
\endgroup
\caption{STM: results} 
\label{tab:stm.results}
\end{table}


==> Tables/junk/table_ATE.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu Oct 24 13:46:45 2019
\begin{table}[H]
\centering
\begingroup\scriptsize
\begin{tabular}{lrrrr}
  \toprule
 & Estimate & Std. Error & t value & Pr($>$$|$t$|$) \\ 
  \midrule
Control vs. ISF & -0.4030847 & 0.03375392 & -11.9418629 & 0.0000000 \\ 
  Control vs. LEGA & -0.0209770 & 0.02404345 & -0.8724614 & 0.3829686 \\ 
  Control vs. LEGA.ISF & -0.4949699 & 0.14079458 & -3.5155465 & 0.0004400 \\ 
  Control vs. LEGA.LOGO & -0.1805311 & 0.13868393 & -1.3017449 & 0.1930206 \\ 
  Control vs. LOGO & -0.2671383 & 0.05008892 & -5.3332807 & 0.0000001 \\ 
  Control vs. LOGO.ISF & -0.3536888 & 0.08922044 & -3.9642130 & 0.0000739 \\ 
  LOGO vs LEGA & -0.2461613 & 0.05350226 & -4.6009511 & 0.0000042 \\ 
  LOGO vs ISF & 0.1359464 & 0.05851267 & 2.3233669 & 0.0201708 \\ 
  LEGA vs ISF & 0.3821077 & 0.03863831 & 9.8893475 & 0.0000000 \\ 
   \bottomrule
\end{tabular}
\endgroup
\caption{ATE pair-wise estimation} 
\label{tab:ATE}
\end{table}


==> Tables/junk/table_ATET.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu Dec 05 11:25:01 2019
\begin{table}
\centering
\begingroup\normalfont
\begin{tabular}{lrrrr}
  \toprule
Pairwise ATET & estimate & std.error & statistic & p.value \\ 
  \midrule
  KK - ISF & -0.89 & 0.05 & -16.43 & 0.00 \\ 
  ISF - KK & 0.83 & 0.05 & 17.33 & 0.00 \\ 
  %ISF - SON & 0.09 & 0.09 & 1.02 & 0.31 \\ 
  %SON - ISF & -0.04 & 0.11 & -0.40 & 0.69 \\ 
  %KK - SON & -0.84 & 0.10 & -8.53 & 0.00 \\ 
  %SON - KK & 0.81 & 0.11 & 7.05 & 0.00 \\ 
   \bottomrule
\end{tabular}
\endgroup
\caption{ATET pair-wise estimation on the SW8 score for math and language} 
\label{table:ATET}
\end{table}


==> Tables/junk/therapy_rs.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Sun, Jan 19, 2020 - 12:37:11 PM
\begin{table}[h!] \centering 
  \caption{RS} 
  \label{table:rs_treat} 
\footnotesize 
\begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{7}{c}{\textit{Dependent variable:}} \\ 
\cline{2-8} 
\\[-1.8ex] & OTHER & LEGA & ISF & LOGO & DYSK & KK & SON \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7)\\ 
\hline \\[-1.8ex] 
 regionalstelleGossau & $-$0.06$^{***}$ & 0.12$^{***}$ & $-$0.01 & $-$0.06$^{***}$ & $-$0.01$^{*}$ & $-$0.004 & 0.003 \\ 
  & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.005) & (0.003) \\ 
  regionalstelleWil & $-$0.04$^{***}$ & 0.02$^{**}$ & 0.05$^{***}$ & $-$0.03$^{***}$ & 0.01$^{*}$ & 0.002 & $-$0.003 \\ 
  & (0.01) & (0.01) & (0.01) & (0.01) & (0.005) & (0.004) & (0.003) \\ 
  regionalstelleWattwil & $-$0.02 & 0.01 & 0.07$^{***}$ & $-$0.05$^{***}$ & $-$0.002 & $-$0.03$^{***}$ & 0.003 \\ 
  & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.004) & (0.003) \\ 
  regionalstelleRapperswil-Jona & $-$0.03$^{***}$ & $-$0.05$^{***}$ & 0.19$^{***}$ & $-$0.09$^{***}$ & $-$0.03$^{***}$ & $-$0.02$^{***}$ & $-$0.0000 \\ 
  & (0.01) & (0.01) & (0.01) & (0.01) & (0.005) & (0.004) & (0.003) \\ 
  regionalstelleSargans & 0.01 & 0.01 & 0.07$^{***}$ & $-$0.09$^{***}$ & 0.01$^{*}$ & $-$0.01$^{**}$ & $-$0.01$^{**}$ \\ 
  & (0.01) & (0.01) & (0.01) & (0.01) & (0.005) & (0.004) & (0.003) \\ 
  regionalstelleRebstein & 0.01 & 0.03$^{***}$ & 0.01$^{**}$ & $-$0.05$^{***}$ & $-$0.001 & $-$0.001 & $-$0.001 \\ 
  & (0.01) & (0.01) & (0.01) & (0.01) & (0.005) & (0.004) & (0.003) \\ 
  Constant & 0.90$^{***}$ & 0.05$^{***}$ & $-$0.12$^{***}$ & 0.21$^{***}$ & $-$0.02$^{***}$ & $-$0.01$^{*}$ & 0.02$^{***}$ \\ 
  & (0.02) & (0.01) & (0.01) & (0.01) & (0.01) & (0.01) & (0.004) \\ 
 \hline \\[-1.8ex] 
Individual characteristics & Yes & Yes & Yes & Yes & Yes &  &  \\ 
Year FE & Yes & Yes & Yes & Yes & Yes &  &  \\ 
Observations & 25'350 & 25'350 & 25'350 & 25'350 & 25'350 & 25'350 & 25'350 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{7}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Tables/junk/therapy_year.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Dec 20, 2019 - 9:39:01 AM
\begin{table}[h!] \centering 
  \caption{Unconditional and conditional comparison of assigned therapies over time} 
  \label{table:year_treat} 
\footnotesize 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
\\[-1.8ex] & OTHER & LEGA & ISF & LOGO & DYSK & KK \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 Year 2000 & 0.77$^{***}$ & 0.02$^{***}$ & 0.02$^{*}$ &  &  &  \\ 
  & (0.02) & (0.01) & (0.01) &  &  &  \\ 
  Year 2001 & 0.71$^{***}$ & 0.02$^{***}$ & 0.04$^{***}$ & $-$0.04 & $-$0.0001 & 0.01 \\ 
  & (0.02) & (0.01) & (0.01) & (0.02) & (0.01) & (0.01) \\ 
  Year 2002 & 0.62$^{***}$ & 0.03$^{***}$ & 0.04$^{***}$ & $-$0.09$^{***}$ & 0.01 & 0.01 \\ 
  & (0.01) & (0.005) & (0.01) & (0.02) & (0.01) & (0.01) \\ 
  Year 2003 & 0.61$^{***}$ & 0.03$^{***}$ & 0.05$^{***}$ & $-$0.08$^{***}$ & $-$0.001 & 0.01 \\ 
  & (0.01) & (0.004) & (0.01) & (0.02) & (0.01) & (0.01) \\ 
  Year 2004 & 0.59$^{***}$ & 0.03$^{***}$ & 0.06$^{***}$ & $-$0.09$^{***}$ & $-$0.01 & 0.02 \\ 
  & (0.01) & (0.004) & (0.01) & (0.02) & (0.01) & (0.01) \\ 
  Year 2005 & 0.56$^{***}$ & 0.03$^{***}$ & 0.08$^{***}$ & $-$0.11$^{***}$ & $-$0.005 & 0.03$^{**}$ \\ 
  & (0.01) & (0.004) & (0.01) & (0.02) & (0.01) & (0.01) \\ 
  Year 2006 & 0.58$^{***}$ & 0.03$^{***}$ & 0.08$^{***}$ & $-$0.08$^{***}$ & $-$0.01$^{*}$ & 0.03$^{**}$ \\ 
  & (0.01) & (0.004) & (0.01) & (0.02) & (0.01) & (0.01) \\ 
  Year 2007 & 0.57$^{***}$ & 0.03$^{***}$ & 0.09$^{***}$ & $-$0.09$^{***}$ & $-$0.01$^{*}$ & 0.04$^{***}$ \\ 
  & (0.01) & (0.004) & (0.01) & (0.02) & (0.01) & (0.01) \\ 
  Year 2008 & 0.55$^{***}$ & 0.02$^{***}$ & 0.13$^{***}$ & $-$0.10$^{***}$ & $-$0.02$^{***}$ & 0.07$^{***}$ \\ 
  & (0.01) & (0.003) & (0.01) & (0.02) & (0.01) & (0.01) \\ 
  Year 2009 & 0.48$^{***}$ & 0.03$^{***}$ & 0.16$^{***}$ & $-$0.13$^{***}$ & $-$0.02$^{**}$ & 0.10$^{***}$ \\ 
  & (0.01) & (0.004) & (0.01) & (0.02) & (0.01) & (0.01) \\ 
  as.factor(year.school)2009-10 & 0.46$^{***}$ & 0.04$^{***}$ & 0.15$^{***}$ & $-$0.13$^{***}$ & $-$0.02 & 0.08$^{***}$ \\ 
  & (0.02) & (0.01) & (0.01) & (0.03) & (0.01) & (0.02) \\ 
  Constant &  &  &  & 1.04$^{***}$ & $-$0.04$^{***}$ & $-$0.14$^{***}$ \\ 
  &  &  &  & (0.03) & (0.01) & (0.02) \\ 
 \hline \\[-1.8ex] 
Characteristics & No & No & No & No & No & Yes \\ 
Observations & 16'106 & 16'106 & 16'106 & 16'106 & 16'106 & 16'106 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Tables/junk/year_treat.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Feb 20, 2020 - 4:53:26 PM
\begin{table}[h!] \centering 
  \caption{Unconditional and conditional comparison of assigned therapies over time} 
  \label{table:year_treat} 
\footnotesize 
\begin{tabular}{@{\extracolsep{5pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{\textit{Dependent variable:}} \\ 
\cline{2-7} 
\\[-1.8ex] & OTHER & KK & ISF & OTHER & KK & ISF \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 School year 2000 & 0.73$^{***}$ & 0.03$^{***}$ & 0.03$^{**}$ &  &  &  \\ 
  & (0.02) & (0.01) & (0.01) &  &  &  \\ 
  School year 2001 & 0.68$^{***}$ & 0.02$^{***}$ & 0.04$^{***}$ & $-$0.03 & $-$0.01 & 0.01 \\ 
  & (0.01) & (0.005) & (0.01) & (0.02) & (0.01) & (0.01) \\ 
  School year 2002 & 0.61$^{***}$ & 0.03$^{***}$ & 0.05$^{***}$ & $-$0.09$^{***}$ & $-$0.004 & 0.01 \\ 
  & (0.01) & (0.004) & (0.01) & (0.02) & (0.01) & (0.01) \\ 
  School year 2003 & 0.60$^{***}$ & 0.03$^{***}$ & 0.05$^{***}$ & $-$0.08$^{***}$ & $-$0.01$^{*}$ & 0.01 \\ 
  & (0.01) & (0.004) & (0.01) & (0.02) & (0.01) & (0.01) \\ 
  School year 2004 & 0.56$^{***}$ & 0.02$^{***}$ & 0.07$^{***}$ & $-$0.10$^{***}$ & $-$0.02$^{***}$ & 0.02$^{*}$ \\ 
  & (0.01) & (0.004) & (0.01) & (0.02) & (0.01) & (0.01) \\ 
  School year 2005 & 0.52$^{***}$ & 0.03$^{***}$ & 0.09$^{***}$ & $-$0.12$^{***}$ & $-$0.01$^{**}$ & 0.04$^{***}$ \\ 
  & (0.01) & (0.004) & (0.01) & (0.02) & (0.01) & (0.01) \\ 
  School year 2006 & 0.54$^{***}$ & 0.03$^{***}$ & 0.10$^{***}$ & $-$0.09$^{***}$ & $-$0.02$^{***}$ & 0.04$^{***}$ \\ 
  & (0.01) & (0.004) & (0.01) & (0.02) & (0.01) & (0.01) \\ 
  School year 2007 & 0.54$^{***}$ & 0.02$^{***}$ & 0.10$^{***}$ & $-$0.10$^{***}$ & $-$0.02$^{***}$ & 0.04$^{***}$ \\ 
  & (0.01) & (0.003) & (0.01) & (0.02) & (0.01) & (0.01) \\ 
  School year 2008 & 0.52$^{***}$ & 0.02$^{***}$ & 0.14$^{***}$ & $-$0.13$^{***}$ & $-$0.03$^{***}$ & 0.08$^{***}$ \\ 
  & (0.01) & (0.003) & (0.01) & (0.02) & (0.01) & (0.01) \\ 
  School year 2009 & 0.50$^{***}$ & 0.02$^{***}$ & 0.15$^{***}$ & $-$0.14$^{***}$ & $-$0.03$^{***}$ & 0.09$^{***}$ \\ 
  & (0.01) & (0.003) & (0.01) & (0.02) & (0.01) & (0.01) \\ 
  School year 2010 & 0.44$^{***}$ & 0.03$^{***}$ & 0.15$^{***}$ & $-$0.18$^{***}$ & $-$0.03$^{***}$ & 0.10$^{***}$ \\ 
  & (0.02) & (0.01) & (0.01) & (0.03) & (0.01) & (0.02) \\ 
  Constant &  &  &  & 1.15$^{***}$ & $-$0.03$^{***}$ & $-$0.15$^{***}$ \\ 
  &  &  &  & (0.03) & (0.01) & (0.01) \\ 
 \hline \\[-1.8ex] 
Characteristics & No & No & No & Yes & Yes & Yes \\ 
Observations & 18'017 & 18'017 & 18'017 & 18'017 & 18'017 & 18'017 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> Tables/main.tex <==

\begin{ThreePartTable}
\centering
\begin{TableNotes}
\item \textit{Note: } 
\item Coefficients in bold are statistically significant at the 95\% level.
\end{TableNotes}
\begin{longtable}[t]{llcccc}
\caption{Main results \label{table:main}}\\
\toprule
\multicolumn{1}{c}{ } & \multicolumn{5}{c}{Estimates} \\
\cmidrule(l{3pt}r{3pt}){2-6}
Pairwise effect & Estimand & Point estimate & Standard error & Conf. int. low & Conf. int. high\\
\midrule
\endfirsthead
\caption[]{Main results \label{table:main} \textit{(continued)}}\\
\toprule
\multicolumn{1}{c}{ } & \multicolumn{5}{c}{Estimates} \\
\cmidrule(l{3pt}r{3pt}){2-6}
Pairwise effect & Estimand & Point estimate & Standard error & Conf. int. low & Conf. int. high\\
\midrule
\endhead

\endfoot
\bottomrule
\insertTableNotes
\endlastfoot
\addlinespace[1em]
\multicolumn{6}{l}{\textbf{SW8 test results}}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{-0.141}} & \cellcolor{gray!6}{3.273} & \cellcolor{gray!6}{-0.205} & \cellcolor{gray!6}{-0.077}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{-0.183}} & \cellcolor{gray!6}{3.296} & \cellcolor{gray!6}{-0.262} & \cellcolor{gray!6}{-0.105}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{-0.078} & \cellcolor{gray!6}{0.040} & \cellcolor{gray!6}{-0.157} & \cellcolor{gray!6}{0.001}\\
\hspace{1em}ISF-None & ATE & \textbf{-0.378} & 3.741 & -0.451 & -0.305\\
\hspace{1em}ISF-None & ATET & \textbf{-1.006} & 4.263 & -1.132 & -0.880\\
\hspace{1em}ISF-None & ATO & \textbf{-0.342} & 0.047 & -0.435 & -0.249\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{-0.617}} & \cellcolor{gray!6}{5.160} & \cellcolor{gray!6}{-0.718} & \cellcolor{gray!6}{-0.516}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{-2.111}} & \cellcolor{gray!6}{6.642} & \cellcolor{gray!6}{-2.358} & \cellcolor{gray!6}{-1.864}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{-0.623}} & \cellcolor{gray!6}{0.059} & \cellcolor{gray!6}{-0.740} & \cellcolor{gray!6}{-0.507}\\
\hspace{1em}KK-None & ATE & \textbf{-0.994} & 5.533 & -1.102 & -0.887\\
\hspace{1em}KK-None & ATET & \textbf{-2.702} & 9.552 & -3.024 & -2.379\\
\hspace{1em}KK-None & ATO & \textbf{-0.965} & 0.062 & -1.086 & -0.844\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{0.572}} & \cellcolor{gray!6}{8.306} & \cellcolor{gray!6}{0.411} & \cellcolor{gray!6}{0.734}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{4.207}} & \cellcolor{gray!6}{14.185} & \cellcolor{gray!6}{3.457} & \cellcolor{gray!6}{4.956}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{0.568}} & \cellcolor{gray!6}{0.086} & \cellcolor{gray!6}{0.399} & \cellcolor{gray!6}{0.737}\\
\hspace{1em}SON-None & ATE & \textbf{-0.422} & 7.505 & -0.568 & -0.276\\
\hspace{1em}SON-None & ATET & \textbf{-1.225} & 9.115 & -1.552 & -0.899\\
\hspace{1em}SON-None & ATO & \textbf{-0.397} & 0.079 & -0.551 & -0.243\\
\addlinespace[1em]
\multicolumn{6}{l}{\textbf{Probability of being unemployed}}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{-0.016} & \cellcolor{gray!6}{1.655} & \cellcolor{gray!6}{-0.044} & \cellcolor{gray!6}{0.011}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{-0.025} & \cellcolor{gray!6}{1.919} & \cellcolor{gray!6}{-0.062} & \cellcolor{gray!6}{0.011}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{-0.013} & \cellcolor{gray!6}{0.019} & \cellcolor{gray!6}{-0.049} & \cellcolor{gray!6}{0.023}\\
\hspace{1em}ISF-None & ATE & 0.005 & 2.711 & -0.040 & 0.049\\
\hspace{1em}ISF-None & ATET & 0.035 & 2.214 & -0.018 & 0.088\\
\hspace{1em}ISF-None & ATO & 0.006 & 0.026 & -0.044 & 0.057\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{0.124}} & \cellcolor{gray!6}{3.625} & \cellcolor{gray!6}{0.065} & \cellcolor{gray!6}{0.184}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{0.508}} & \cellcolor{gray!6}{4.165} & \cellcolor{gray!6}{0.354} & \cellcolor{gray!6}{0.661}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{0.096}} & \cellcolor{gray!6}{0.031} & \cellcolor{gray!6}{0.035} & \cellcolor{gray!6}{0.157}\\
\hspace{1em}KK-None & ATE & \textbf{0.129} & 3.122 & 0.078 & 0.180\\
\hspace{1em}KK-None & ATET & \textbf{0.208} & 3.517 & 0.122 & 0.294\\
\hspace{1em}KK-None & ATO & \textbf{0.102} & 0.028 & 0.048 & 0.156\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{-0.136}} & \cellcolor{gray!6}{4.274} & \cellcolor{gray!6}{-0.206} & \cellcolor{gray!6}{-0.066}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{-0.476}} & \cellcolor{gray!6}{5.030} & \cellcolor{gray!6}{-0.679} & \cellcolor{gray!6}{-0.272}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{-0.1}} & \cellcolor{gray!6}{0.036} & \cellcolor{gray!6}{-0.170} & \cellcolor{gray!6}{-0.031}\\
\hspace{1em}SON-None & ATE & -0.007 & 3.533 & -0.065 & 0.051\\
\hspace{1em}SON-None & ATET & -0.018 & 4.092 & -0.120 & 0.085\\
\hspace{1em}SON-None & ATO & 0.002 & 0.031 & -0.060 & 0.063\\
\addlinespace[1em]
\multicolumn{6}{l}{\textbf{Probability of using DI}}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{-0.031}} & \cellcolor{gray!6}{1.211} & \cellcolor{gray!6}{-0.051} & \cellcolor{gray!6}{-0.011}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{-0.021}} & \cellcolor{gray!6}{1.031} & \cellcolor{gray!6}{-0.041} & \cellcolor{gray!6}{-0.001}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{-0.05}} & \cellcolor{gray!6}{0.016} & \cellcolor{gray!6}{-0.081} & \cellcolor{gray!6}{-0.019}\\
\hspace{1em}ISF-None & ATE & -0.014 & 2.336 & -0.052 & 0.025\\
\hspace{1em}ISF-None & ATET & \textbf{-0.034} & 1.017 & -0.058 & -0.009\\
\hspace{1em}ISF-None & ATO & -0.035 & 0.021 & -0.077 & 0.007\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{0.011} & \cellcolor{gray!6}{2.583} & \cellcolor{gray!6}{-0.031} & \cellcolor{gray!6}{0.054}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{0.087} & \cellcolor{gray!6}{2.478} & \cellcolor{gray!6}{-0.004} & \cellcolor{gray!6}{0.179}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{0.023} & \cellcolor{gray!6}{0.022} & \cellcolor{gray!6}{-0.021} & \cellcolor{gray!6}{0.067}\\
\hspace{1em}KK-None & ATE & -0.002 & 1.932 & -0.034 & 0.029\\
\hspace{1em}KK-None & ATET & 0.012 & 1.933 & -0.036 & 0.059\\
\hspace{1em}KK-None & ATO & -0.013 & 0.022 & -0.055 & 0.030\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{0.12}} & \cellcolor{gray!6}{3.548} & \cellcolor{gray!6}{0.061} & \cellcolor{gray!6}{0.178}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{0.717}} & \cellcolor{gray!6}{5.336} & \cellcolor{gray!6}{0.501} & \cellcolor{gray!6}{0.933}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{0.11}} & \cellcolor{gray!6}{0.029} & \cellcolor{gray!6}{0.052} & \cellcolor{gray!6}{0.167}\\
\hspace{1em}SON-None & ATE & \textbf{0.117} & 3.372 & 0.062 & 0.173\\
\hspace{1em}SON-None & ATET & 0.126 & 5.926 & -0.022 & 0.275\\
\hspace{1em}SON-None & ATO & \textbf{0.097} & 0.029 & 0.041 & 0.153\\
\addlinespace[1em]
\multicolumn{6}{l}{\textbf{Work income (month)}}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{0.132}} & \cellcolor{gray!6}{3.574} & \cellcolor{gray!6}{0.073} & \cellcolor{gray!6}{0.191}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{0.11}} & \cellcolor{gray!6}{4.347} & \cellcolor{gray!6}{0.027} & \cellcolor{gray!6}{0.194}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{0.152}} & \cellcolor{gray!6}{0.039} & \cellcolor{gray!6}{0.076} & \cellcolor{gray!6}{0.228}\\
\hspace{1em}ISF-None & ATE & 0.076 & 5.716 & -0.018 & 0.170\\
\hspace{1em}ISF-None & ATET & \textbf{0.174} & 5.241 & 0.047 & 0.300\\
\hspace{1em}ISF-None & ATO & 0.08 & 0.053 & -0.023 & 0.183\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{-0.211}} & \cellcolor{gray!6}{7.311} & \cellcolor{gray!6}{-0.331} & \cellcolor{gray!6}{-0.091}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{-0.37}} & \cellcolor{gray!6}{7.520} & \cellcolor{gray!6}{-0.647} & \cellcolor{gray!6}{-0.093}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{-0.169}} & \cellcolor{gray!6}{0.061} & \cellcolor{gray!6}{-0.289} & \cellcolor{gray!6}{-0.050}\\
\hspace{1em}KK-None & ATE & \textbf{-0.135} & 6.229 & -0.237 & -0.033\\
\hspace{1em}KK-None & ATET & 0.035 & 6.421 & -0.122 & 0.192\\
\hspace{1em}KK-None & ATO & -0.089 & 0.056 & -0.198 & 0.020\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{-0.057} & \cellcolor{gray!6}{10.954} & \cellcolor{gray!6}{-0.237} & \cellcolor{gray!6}{0.123}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{-1.309}} & \cellcolor{gray!6}{10.546} & \cellcolor{gray!6}{-1.736} & \cellcolor{gray!6}{-0.883}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{-0.14} & \cellcolor{gray!6}{0.077} & \cellcolor{gray!6}{-0.291} & \cellcolor{gray!6}{0.010}\\
\hspace{1em}SON-None & ATE & \textbf{-0.192} & 9.960 & -0.355 & -0.029\\
\hspace{1em}SON-None & ATET & \textbf{-0.484} & 8.937 & -0.708 & -0.260\\
\hspace{1em}SON-None & ATO & \textbf{-0.23} & 0.070 & -0.368 & -0.092\\*
\end{longtable}
\end{ThreePartTable}


==> Tables/main_CS.tex <==

\begin{ThreePartTable}
\begin{TableNotes}
\item \textit{Note: } 
\item Coefficients in bold are statistically significant at the 95\% level.
\end{TableNotes}
\begin{longtable}[t]{llcccc}
\caption{\label{tab:}Main results: CS \label{table:main}}\\
\toprule
\multicolumn{1}{c}{ } & \multicolumn{5}{c}{Estimates} \\
\cmidrule(l{3pt}r{3pt}){2-6}
Pairwise effect & Estimand & Point estimate & Standard error & Conf. int. low & Conf. int. high\\
\midrule
\endfirsthead
\caption[]{Main results: CS \label{table:main} \textit{(continued)}}\\
\toprule
\multicolumn{1}{c}{ } & \multicolumn{5}{c}{Estimates} \\
\cmidrule(l{3pt}r{3pt}){2-6}
Pairwise effect & Estimand & Point estimate & Standard error & Conf. int. low & Conf. int. high\\
\midrule
\endhead

\endfoot
\bottomrule
\insertTableNotes
\endlastfoot
\addlinespace[1em]
\multicolumn{6}{l}{\textbf{SW8 test results}}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{-0.162}} & \cellcolor{gray!6}{2.238} & \cellcolor{gray!6}{-0.210} & \cellcolor{gray!6}{-0.114}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{-0.123}} & \cellcolor{gray!6}{2.450} & \cellcolor{gray!6}{-0.175} & \cellcolor{gray!6}{-0.071}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{-0.072} & \cellcolor{gray!6}{0.042} & \cellcolor{gray!6}{-0.155} & \cellcolor{gray!6}{0.010}\\
\hspace{1em}ISF-None & ATE & \textbf{-0.391} & 2.390 & -0.442 & -0.340\\
\hspace{1em}ISF-None & ATET & \textbf{-0.452} & 4.019 & -0.537 & -0.366\\
\hspace{1em}ISF-None & ATO & \textbf{-0.342} & 0.050 & -0.440 & -0.245\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{-0.588}} & \cellcolor{gray!6}{2.318} & \cellcolor{gray!6}{-0.637} & \cellcolor{gray!6}{-0.538}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{-0.574}} & \cellcolor{gray!6}{3.650} & \cellcolor{gray!6}{-0.652} & \cellcolor{gray!6}{-0.496}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{-0.623}} & \cellcolor{gray!6}{0.061} & \cellcolor{gray!6}{-0.743} & \cellcolor{gray!6}{-0.503}\\
\hspace{1em}KK-None & ATE & \textbf{-0.979} & 2.719 & -1.037 & -0.921\\
\hspace{1em}KK-None & ATET & \textbf{-0.794} & 8.080 & -0.966 & -0.622\\
\hspace{1em}KK-None & ATO & \textbf{-0.966} & 0.063 & -1.090 & -0.841\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{0.656}} & \cellcolor{gray!6}{2.170} & \cellcolor{gray!6}{0.610} & \cellcolor{gray!6}{0.703}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{0.59}} & \cellcolor{gray!6}{7.954} & \cellcolor{gray!6}{0.420} & \cellcolor{gray!6}{0.760}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{0.563}} & \cellcolor{gray!6}{0.087} & \cellcolor{gray!6}{0.392} & \cellcolor{gray!6}{0.734}\\
\hspace{1em}SON-None & ATE & \textbf{-0.323} & 2.245 & -0.371 & -0.275\\
\hspace{1em}SON-None & ATET & \textbf{-0.304} & 6.120 & -0.435 & -0.174\\
\hspace{1em}SON-None & ATO & \textbf{-0.403} & 0.080 & -0.559 & -0.247\\
\addlinespace[1em]
\multicolumn{6}{l}{\textbf{Probability of being unemployed}}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{-0.012} & \cellcolor{gray!6}{1.321} & \cellcolor{gray!6}{-0.037} & \cellcolor{gray!6}{0.012}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{-0.021} & \cellcolor{gray!6}{1.710} & \cellcolor{gray!6}{-0.053} & \cellcolor{gray!6}{0.011}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{-0.011} & \cellcolor{gray!6}{0.020} & \cellcolor{gray!6}{-0.050} & \cellcolor{gray!6}{0.029}\\
\hspace{1em}ISF-None & ATE & 0.003 & 1.638 & -0.027 & 0.034\\
\hspace{1em}ISF-None & ATET & 0.026 & 1.930 & -0.009 & 0.062\\
\hspace{1em}ISF-None & ATO & 0.007 & 0.027 & -0.046 & 0.060\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{0.106}} & \cellcolor{gray!6}{1.820} & \cellcolor{gray!6}{0.072} & \cellcolor{gray!6}{0.140}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{0.103}} & \cellcolor{gray!6}{2.156} & \cellcolor{gray!6}{0.062} & \cellcolor{gray!6}{0.143}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{0.092}} & \cellcolor{gray!6}{0.032} & \cellcolor{gray!6}{0.030} & \cellcolor{gray!6}{0.154}\\
\hspace{1em}KK-None & ATE & \textbf{0.109} & 1.835 & 0.075 & 0.143\\
\hspace{1em}KK-None & ATET & \textbf{0.085} & 3.180 & 0.026 & 0.145\\
\hspace{1em}KK-None & ATO & \textbf{0.099} & 0.029 & 0.042 & 0.156\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{-0.106}} & \cellcolor{gray!6}{1.687} & \cellcolor{gray!6}{-0.138} & \cellcolor{gray!6}{-0.075}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{-0.066} & \cellcolor{gray!6}{3.652} & \cellcolor{gray!6}{-0.134} & \cellcolor{gray!6}{0.002}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{-0.085}} & \cellcolor{gray!6}{0.037} & \cellcolor{gray!6}{-0.157} & \cellcolor{gray!6}{-0.013}\\
\hspace{1em}SON-None & ATE & 0.003 & 1.488 & -0.025 & 0.030\\
\hspace{1em}SON-None & ATET & -0.01 & 3.836 & -0.081 & 0.062\\
\hspace{1em}SON-None & ATO & 0.014 & 0.033 & -0.050 & 0.078\\
\addlinespace[1em]
\multicolumn{6}{l}{\textbf{Probability of using DI}}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{-0.028}} & \cellcolor{gray!6}{1.024} & \cellcolor{gray!6}{-0.047} & \cellcolor{gray!6}{-0.009}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{-0.019}} & \cellcolor{gray!6}{0.942} & \cellcolor{gray!6}{-0.037} & \cellcolor{gray!6}{-0.001}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{-0.053}} & \cellcolor{gray!6}{0.017} & \cellcolor{gray!6}{-0.087} & \cellcolor{gray!6}{-0.020}\\
\hspace{1em}ISF-None & ATE & -0.012 & 1.438 & -0.039 & 0.014\\
\hspace{1em}ISF-None & ATET & -0.015 & 0.852 & -0.031 & 0.001\\
\hspace{1em}ISF-None & ATO & -0.036 & 0.023 & -0.080 & 0.009\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{0.009} & \cellcolor{gray!6}{1.335} & \cellcolor{gray!6}{-0.016} & \cellcolor{gray!6}{0.034}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{0.016} & \cellcolor{gray!6}{1.363} & \cellcolor{gray!6}{-0.009} & \cellcolor{gray!6}{0.041}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{0.021} & \cellcolor{gray!6}{0.023} & \cellcolor{gray!6}{-0.025} & \cellcolor{gray!6}{0.066}\\
\hspace{1em}KK-None & ATE & -0.003 & 1.246 & -0.026 & 0.020\\
\hspace{1em}KK-None & ATET & 0.001 & 1.663 & -0.030 & 0.032\\
\hspace{1em}KK-None & ATO & -0.015 & 0.023 & -0.060 & 0.030\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{0.11}} & \cellcolor{gray!6}{1.202} & \cellcolor{gray!6}{0.088} & \cellcolor{gray!6}{0.133}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{0.101}} & \cellcolor{gray!6}{3.812} & \cellcolor{gray!6}{0.030} & \cellcolor{gray!6}{0.172}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{0.111}} & \cellcolor{gray!6}{0.030} & \cellcolor{gray!6}{0.052} & \cellcolor{gray!6}{0.171}\\
\hspace{1em}SON-None & ATE & \textbf{0.107} & 1.316 & 0.082 & 0.131\\
\hspace{1em}SON-None & ATET & -0.017 & 6.089 & -0.130 & 0.096\\
\hspace{1em}SON-None & ATO & \textbf{0.096} & 0.030 & 0.038 & 0.155\\
\addlinespace[1em]
\multicolumn{6}{l}{\textbf{Work income (month)}}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{0.136}} & \cellcolor{gray!6}{2.822} & \cellcolor{gray!6}{0.083} & \cellcolor{gray!6}{0.188}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{0.088}} & \cellcolor{gray!6}{3.838} & \cellcolor{gray!6}{0.017} & \cellcolor{gray!6}{0.160}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{0.159}} & \cellcolor{gray!6}{0.042} & \cellcolor{gray!6}{0.076} & \cellcolor{gray!6}{0.241}\\
\hspace{1em}ISF-None & ATE & \textbf{0.066} & 3.522 & 0.001 & 0.132\\
\hspace{1em}ISF-None & ATET & 0.067 & 4.312 & -0.013 & 0.148\\
\hspace{1em}ISF-None & ATO & 0.079 & 0.056 & -0.030 & 0.189\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{-0.129}} & \cellcolor{gray!6}{3.706} & \cellcolor{gray!6}{-0.198} & \cellcolor{gray!6}{-0.060}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{-0.046} & \cellcolor{gray!6}{4.009} & \cellcolor{gray!6}{-0.121} & \cellcolor{gray!6}{0.029}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{-0.156}} & \cellcolor{gray!6}{0.063} & \cellcolor{gray!6}{-0.279} & \cellcolor{gray!6}{-0.032}\\
\hspace{1em}KK-None & ATE & -0.063 & 3.694 & -0.132 & 0.006\\
\hspace{1em}KK-None & ATET & 0.068 & 5.605 & -0.036 & 0.172\\
\hspace{1em}KK-None & ATO & -0.077 & 0.058 & -0.191 & 0.038\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{-0.13}} & \cellcolor{gray!6}{3.862} & \cellcolor{gray!6}{-0.202} & \cellcolor{gray!6}{-0.058}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{-0.163}} & \cellcolor{gray!6}{7.353} & \cellcolor{gray!6}{-0.300} & \cellcolor{gray!6}{-0.026}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{-0.155}} & \cellcolor{gray!6}{0.079} & \cellcolor{gray!6}{-0.310} & \cellcolor{gray!6}{-0.001}\\
\hspace{1em}SON-None & ATE & \textbf{-0.193} & 3.685 & -0.261 & -0.124\\
\hspace{1em}SON-None & ATET & \textbf{-0.177} & 8.498 & -0.335 & -0.019\\
\hspace{1em}SON-None & ATO & \textbf{-0.232} & 0.073 & -0.376 & -0.088\\*
\end{longtable}
\end{ThreePartTable}


==> Tables/main_FULL.tex <==

\begin{ThreePartTable}
\begin{TableNotes}
\item \textit{Note: } 
\item Coefficients in bold are statistically significant at the 95\% level.
\end{TableNotes}
\begin{longtable}[t]{llcccc}
\caption{\label{tab:}Main results: FULL \label{table:main}}\\
\toprule
\multicolumn{1}{c}{ } & \multicolumn{5}{c}{Estimates} \\
\cmidrule(l{3pt}r{3pt}){2-6}
Pairwise effect & Estimand & Point estimate & Standard error & Conf. int. low & Conf. int. high\\
\midrule
\endfirsthead
\caption[]{Main results: FULL \label{table:main} \textit{(continued)}}\\
\toprule
\multicolumn{1}{c}{ } & \multicolumn{5}{c}{Estimates} \\
\cmidrule(l{3pt}r{3pt}){2-6}
Pairwise effect & Estimand & Point estimate & Standard error & Conf. int. low & Conf. int. high\\
\midrule
\endhead

\endfoot
\bottomrule
\insertTableNotes
\endlastfoot
\addlinespace[1em]
\multicolumn{6}{l}{\textbf{SW8 test results}}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{-0.07} & \cellcolor{gray!6}{8.777} & \cellcolor{gray!6}{-0.239} & \cellcolor{gray!6}{0.099}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{-0.086} & \cellcolor{gray!6}{9.158} & \cellcolor{gray!6}{-0.301} & \cellcolor{gray!6}{0.130}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{-0.066} & \cellcolor{gray!6}{0.042} & \cellcolor{gray!6}{-0.147} & \cellcolor{gray!6}{0.016}\\
\hspace{1em}ISF-None & ATE & \textbf{-0.301} & 8.952 & -0.473 & -0.128\\
\hspace{1em}ISF-None & ATET & \textbf{-0.967} & 4.711 & -1.104 & -0.830\\
\hspace{1em}ISF-None & ATO & \textbf{-0.328} & 0.049 & -0.423 & -0.233\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{-0.615}} & \cellcolor{gray!6}{5.133} & \cellcolor{gray!6}{-0.714} & \cellcolor{gray!6}{-0.517}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{-2.015}} & \cellcolor{gray!6}{6.796} & \cellcolor{gray!6}{-2.262} & \cellcolor{gray!6}{-1.768}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{-0.623}} & \cellcolor{gray!6}{0.059} & \cellcolor{gray!6}{-0.739} & \cellcolor{gray!6}{-0.507}\\
\hspace{1em}KK-None & ATE & \textbf{-0.916} & 9.837 & -1.105 & -0.727\\
\hspace{1em}KK-None & ATET & \textbf{-2.284} & 28.007 & -3.221 & -1.347\\
\hspace{1em}KK-None & ATO & \textbf{-0.952} & 0.063 & -1.074 & -0.829\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{0.566}} & \cellcolor{gray!6}{8.262} & \cellcolor{gray!6}{0.407} & \cellcolor{gray!6}{0.725}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{4.161}} & \cellcolor{gray!6}{13.230} & \cellcolor{gray!6}{3.471} & \cellcolor{gray!6}{4.851}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{0.567}} & \cellcolor{gray!6}{0.086} & \cellcolor{gray!6}{0.399} & \cellcolor{gray!6}{0.736}\\
\hspace{1em}SON-None & ATE & \textbf{-0.35} & 11.047 & -0.563 & -0.138\\
\hspace{1em}SON-None & ATET & \textbf{-1.197} & 9.620 & -1.538 & -0.856\\
\hspace{1em}SON-None & ATO & \textbf{-0.384} & 0.079 & -0.539 & -0.229\\
\addlinespace[1em]
\multicolumn{6}{l}{\textbf{Probability of being unemployed}}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{-0.007} & \cellcolor{gray!6}{2.257} & \cellcolor{gray!6}{-0.039} & \cellcolor{gray!6}{0.026}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{3.737} & \cellcolor{gray!6}{-0.061} & \cellcolor{gray!6}{0.060}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{-0.01} & \cellcolor{gray!6}{0.018} & \cellcolor{gray!6}{-0.046} & \cellcolor{gray!6}{0.026}\\
\hspace{1em}ISF-None & ATE & 0.012 & 3.345 & -0.036 & 0.060\\
\hspace{1em}ISF-None & ATET & 0.047 & 2.851 & -0.007 & 0.101\\
\hspace{1em}ISF-None & ATO & 0.009 & 0.026 & -0.041 & 0.059\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{0.128}} & \cellcolor{gray!6}{4.149} & \cellcolor{gray!6}{0.068} & \cellcolor{gray!6}{0.187}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{0.673}} & \cellcolor{gray!6}{5.097} & \cellcolor{gray!6}{0.488} & \cellcolor{gray!6}{0.858}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{0.097}} & \cellcolor{gray!6}{0.031} & \cellcolor{gray!6}{0.036} & \cellcolor{gray!6}{0.157}\\
\hspace{1em}KK-None & ATE & \textbf{0.139} & 3.748 & 0.085 & 0.193\\
\hspace{1em}KK-None & ATET & \textbf{0.255} & 10.125 & 0.061 & 0.448\\
\hspace{1em}KK-None & ATO & \textbf{0.105} & 0.028 & 0.051 & 0.159\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{-0.147}} & \cellcolor{gray!6}{5.427} & \cellcolor{gray!6}{-0.225} & \cellcolor{gray!6}{-0.069}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{-0.608}} & \cellcolor{gray!6}{5.484} & \cellcolor{gray!6}{-0.828} & \cellcolor{gray!6}{-0.388}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{-0.101}} & \cellcolor{gray!6}{0.036} & \cellcolor{gray!6}{-0.170} & \cellcolor{gray!6}{-0.031}\\
\hspace{1em}SON-None & ATE & -0.007 & 4.840 & -0.077 & 0.062\\
\hspace{1em}SON-None & ATET & -0.018 & 4.826 & -0.112 & 0.075\\
\hspace{1em}SON-None & ATO & 0.005 & 0.031 & -0.056 & 0.066\\
\addlinespace[1em]
\multicolumn{6}{l}{\textbf{Probability of using DI}}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{-0.021}} & \cellcolor{gray!6}{1.166} & \cellcolor{gray!6}{-0.037} & \cellcolor{gray!6}{-0.004}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{-0.013} & \cellcolor{gray!6}{1.601} & \cellcolor{gray!6}{-0.039} & \cellcolor{gray!6}{0.014}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{-0.047}} & \cellcolor{gray!6}{0.015} & \cellcolor{gray!6}{-0.077} & \cellcolor{gray!6}{-0.017}\\
\hspace{1em}ISF-None & ATE & -0.005 & 2.450 & -0.040 & 0.030\\
\hspace{1em}ISF-None & ATET & \textbf{-0.025} & 1.230 & -0.049 & -0.002\\
\hspace{1em}ISF-None & ATO & -0.033 & 0.021 & -0.074 & 0.008\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{0.012} & \cellcolor{gray!6}{2.832} & \cellcolor{gray!6}{-0.029} & \cellcolor{gray!6}{0.053}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{0.104} & \cellcolor{gray!6}{3.029} & \cellcolor{gray!6}{-0.006} & \cellcolor{gray!6}{0.214}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{0.023} & \cellcolor{gray!6}{0.022} & \cellcolor{gray!6}{-0.021} & \cellcolor{gray!6}{0.067}\\
\hspace{1em}KK-None & ATE & 0.007 & 2.049 & -0.023 & 0.036\\
\hspace{1em}KK-None & ATET & 0.032 & 3.705 & -0.039 & 0.102\\
\hspace{1em}KK-None & ATO & -0.01 & 0.021 & -0.052 & 0.032\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{0.176}} & \cellcolor{gray!6}{5.520} & \cellcolor{gray!6}{0.097} & \cellcolor{gray!6}{0.256}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{0.964}} & \cellcolor{gray!6}{5.873} & \cellcolor{gray!6}{0.728} & \cellcolor{gray!6}{1.199}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{0.114}} & \cellcolor{gray!6}{0.029} & \cellcolor{gray!6}{0.057} & \cellcolor{gray!6}{0.171}\\
\hspace{1em}SON-None & ATE & \textbf{0.183} & 5.334 & 0.106 & 0.260\\
\hspace{1em}SON-None & ATET & 0.065 & 7.207 & -0.075 & 0.205\\
\hspace{1em}SON-None & ATO & \textbf{0.104} & 0.028 & 0.049 & 0.159\\
\addlinespace[1em]
\multicolumn{6}{l}{\textbf{Work income (month)}}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{0.097}} & \cellcolor{gray!6}{4.519} & \cellcolor{gray!6}{0.032} & \cellcolor{gray!6}{0.162}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{0.053} & \cellcolor{gray!6}{7.501} & \cellcolor{gray!6}{-0.069} & \cellcolor{gray!6}{0.175}\\
\hspace{1em}\cellcolor{gray!6}{Ind. ther.-None} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{0.144}} & \cellcolor{gray!6}{0.038} & \cellcolor{gray!6}{0.069} & \cellcolor{gray!6}{0.219}\\
\hspace{1em}ISF-None & ATE & 0.057 & 6.525 & -0.037 & 0.151\\
\hspace{1em}ISF-None & ATET & \textbf{0.134} & 6.466 & 0.011 & 0.256\\
\hspace{1em}ISF-None & ATO & 0.074 & 0.052 & -0.027 & 0.176\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{\textbf{-0.22}} & \cellcolor{gray!6}{8.128} & \cellcolor{gray!6}{-0.337} & \cellcolor{gray!6}{-0.103}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{-0.495}} & \cellcolor{gray!6}{9.332} & \cellcolor{gray!6}{-0.833} & \cellcolor{gray!6}{-0.157}\\
\hspace{1em}\cellcolor{gray!6}{KK-ISF} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{\textbf{-0.171}} & \cellcolor{gray!6}{0.061} & \cellcolor{gray!6}{-0.290} & \cellcolor{gray!6}{-0.052}\\
\hspace{1em}KK-None & ATE & \textbf{-0.163} & 7.281 & -0.268 & -0.058\\
\hspace{1em}KK-None & ATET & -0.114 & 18.270 & -0.463 & 0.235\\
\hspace{1em}KK-None & ATO & -0.096 & 0.055 & -0.204 & 0.012\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATE} & \cellcolor{gray!6}{-0.146} & \cellcolor{gray!6}{13.827} & \cellcolor{gray!6}{-0.345} & \cellcolor{gray!6}{0.054}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATET} & \cellcolor{gray!6}{\textbf{-1.823}} & \cellcolor{gray!6}{11.642} & \cellcolor{gray!6}{-2.290} & \cellcolor{gray!6}{-1.356}\\
\hspace{1em}\cellcolor{gray!6}{SON-KK} & \cellcolor{gray!6}{ATO} & \cellcolor{gray!6}{-0.147} & \cellcolor{gray!6}{0.077} & \cellcolor{gray!6}{-0.297} & \cellcolor{gray!6}{0.003}\\
\hspace{1em}SON-None & ATE & \textbf{-0.309} & 12.948 & -0.495 & -0.122\\
\hspace{1em}SON-None & ATET & \textbf{-0.359} & 10.522 & -0.563 & -0.154\\
\hspace{1em}SON-None & ATO & \textbf{-0.243} & 0.070 & -0.379 & -0.106\\*
\end{longtable}
\end{ThreePartTable}


==> Tables/optimal.policy.COMPOSITE.tex <==
\begin{table}[p!]
\footnotesize
\centering
\begin{tabular}{lccccc}
\multicolumn{4}{l}{\textbf{Panel A}: Allocation to program in percent and potential cost reduction} \\[1ex]

  \toprule
                                &\% Students    &\% Students        &Policy           &Costs per year      & Percent of   \\ 
                                &sent to        &sent to semi-      &value            &(in mio CHF)        & actual costs   \\ 
                                &inclusion      &segregation        &                 &                    &  \\
  \midrule
\multicolumn{5}{l}{\emph{Overall welfare (70\% academic performance, 30\% labor market integration. N = 1880}} \\[1ex]
\textbf{Actual allocation }       &0.60        &0.40                &-0.005        &40,966          &1      \\
Depth 2 and baseline variables    &0.96        &0.04                &0.175         &37,942          &0.93  \\
Depth 3 and baseline variables    &0.94        &0.06                &0.190         &38,140          &0.93  \\
Depth 2 and diagnosis variables   &0.96        &0.04                &0.175         &37,942          &0.93  \\
Depth 3 and diagnosis variables   &0.94        &0.06                &0.190         &38,140          &0.93 \\
\bottomrule
\end{tabular}


\vspace{10mm}

\begin{tabular}{lccc}
\multicolumn{3}{l}{\textbf{Panel B}: Cross-validated difference between optimal policy value and different policies} \\[1ex]
\toprule
                                  & All inclusion           &All semi-segregation           &Assigned policy \\
\midrule
\multicolumn{3}{l}{\emph{Overall welfare (70\% academic performance, 30\% labor market integration. N = 1880}} \\[1ex]
& \multicolumn{3}{r}{Optimal policies computed on 10-fold cross validation.} \\[1ex]

Depth 2 and baseline variables   &-0.011$^{*}$   &0.515$^{***}$        &0.347$^{***}$     \\
                                 &(0.006)        &(0.044)              &(0.032)    \\
Depth 3 and baseline variables   &-0.013$^{*}$   &0.513$^{***}$        &0.346$^{***}$      \\
                                 &(0.007)        &(0.043)              &(0.032)     \\
Depth 2 and diagnosis variables  &-0.018$^{**}$  &0.509$^{***}$        &0.341$^{***}$      \\
                                 &(0.007)        &(0.043)              &(0.032)     \\
Depth 3 and diagnosis variables  &-0.019$^{**}$  &0.507$^{***}$        &0.339$^{***}$      \\
                                 &(0.009)        &(0.043)              &(0.031)     \\
\bottomrule
& \multicolumn{3}{r}{\emph{Notes:}$^{***}$: p $<$0.01, $^{**}$: p $<$ 0.05, $^{*}$: p $<$ 0.1.} \\
\end{tabular}
\caption{Weighted optimal policies for inclusion and semi-segregation} 
\floatfoot{\textbf{Panel A} of this table shows the treatment assignment from four different policies. The depth indicates the number of tree branches in the policy trees. The baseline variables are individual covariates excluding variables from text, and diagnosis variables are individual covariates + covariates from the diagnoses extracted from the text (dictionary approach). The policy value is the average APO under each policy. Total cost estimates and potential cost reduction from the implemented policies are computed. \textbf{Panel B} displays validation tests to see whether the proposed policies perform better than either sending everyone to inclusion, sending everyone to semi-segregation, or implementing the (already implemented) observed policy using 10-fold cross-validation. For each policy, the average difference between the APO under the optimal policy and the APO under one of the three alternative policies is computed. Inference is done with a one sample $t-$test on the difference.}
\label{table:optimal_policy_COMPOSITE}
\end{table}

==> Tables/outcome.RMSE.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Fri Oct 23 00:28:40 2020
\begin{table}[h]
\centering
\begingroup\scriptsize
\begin{tabular}{llccc}
  \toprule
Outcome & Method  & RMSE (min)  & Number of times  \\ 
        &         &             & best predictor \\
  \midrule
  Probability of using DI & STM, k = 80, with RF & 0.420 & 19\\
  Probability of using DI & STM, k = 10, with RF & 0.420 & 2\\
  Probability of using DI & All, with lasso & 0.421 & 1\\
  Probability of using DI & Text tf and covariates, with RF & 0.422 & 1 \\ 
  Probability of using DI & Word2Vec with 100 word embeddings, with RF & 0.425 & 1 \\ 
  Probability of using DI & Word2Vec with 25 word embeddings, with elastic net & 0.417 & 1 \\ 

  \midrule
  Work income & All, with RF & 0.969 & 9 \\ 
  Work income & Word2Vec 100, with RF & 0.969 & 8 \\ 
  Work income & Word2Vec 25, with RF & 0.965 & 4 \\ 
  Work income & tf-tf-idf, with RF & 0.966 & 2 \\ 
  Work income & STM, k = 10, with RF & 0.978 & 1 \\ 
  Work income & tf-idf, with RF & 0.966 & 1 \\ 
  
  %\midrule
  %Probability of taking the SW8 test & STM, k = 80, with Lasso & 0.369 & 0.371 & 0.364 \\ 
  %Probability of taking the SW8 test & Text tf.tf.idf and covariates, with RF & 0.367 & 0.371 & 0.364 \\ 
  %Probability of taking the SW8 test & Text tf.idf and covariates, with RF & 0.369 & 0.372 & 0.366 \\ 
  %Probability of taking the SW8 test & STM, k = 80, with E.net & 0.369 & 0.371 & 0.364 \\ 
  %Probability of taking the SW8 test & STM, k = 10, with RF & 0.369 & 0.372 & 0.366 \\ 
  
  \midrule
  SW8 test results & No text, with RF  & 0.841 & 20 \\ 
  SW8 test results & STM, k = 80, with RF & 0.854 & 4 \\ 
  SW8 test results & Dictionary dummy 1sd, with RF & 0.844 & 1\\ 

  \midrule
  Probability of being unemployed & STM, k = 10, with RF & 0.403 & 8\\ 
  Probability of being unemployed & Dictionary dummy 0sd, with RF & 0.402 & 7 \\ 
  Probability of being unemployed & Dictionary dummy 1sd, with RF & 0.400 & 3  \\ 
  Probability of being unemployed & tf, with RF & 0.406 & 3 \\ 
  Probability of being unemployed & STM, k = 80, with RF & 0.419 & 2 \\ 
  Probability of being unemployed & Word2Vec100, with lasso & 0.426 & 1 \\ 
  Probability of being unemployed & Word2Vec25, with RF & 0.404 & 1 \\ 
   \bottomrule 
\end{tabular}
\endgroup
\caption{Ensemble learner for outcome} 
\floatfoot{The table summarizes the most predictive methods per fold per treatment. For each fold, for each treatment group, the outcome is predicted, and the method with the lowest RMSE is flagged. For 5 folds and 5 treatment groups, there are 25 winners. Here, the 25 winners are represented. Note that the final predicted score is an ensemble of the most predictive those methods. \emph{Source: SPS}.}
\label{outcome.RMSE}
\end{table}


==> Tables/pscore.RMSE.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Fri Oct 16 15:06:58 2020
\begin{table}[h]
\centering
\begingroup\footnotesize
\begin{tabular}{llccc}
  \toprule
Treatment & Method & RMSE (mean) & RMSE (max) & RMSE (min) \\ 
  \midrule
  Individual therapy & STM and TIRM, with RF                         &0.346     &0.360    &0.329 \\
  Individual therapy & Text tf.tf.idf and covariates, with RF        &0.369     &0.370    &0.366 \\
  Individual therapy & Text tf.idf and covariates, with RF           &0.369     &0.371    &0.365 \\
  Individual therapy & Text tf and covariates, with RF               &0.371     &0.373    &0.369 \\
  Individual therapy & Text tf.idf and covariates, with lasso        &0.375     &0.377    &0.372 \\
   \midrule

  Inclusion           & STM and TIRM, with RF                              &0.161     &0.180    &0.136 \\
  Inclusion           & STM and TIRM, with lasso                           &0.199     &0.219    &0.187 \\
  Inclusion           & TIRM only, with RF                                 &0.202     &0.223    &0.183 \\
  Inclusion           & TIRM only, with lasso                              &0.226     &0.246    &0.211 \\
  Inclusion           & Text tf and covariates, with lasso                 &0.265     &0.271    &0.259 \\
  \midrule
  
  Semi segregation & STM and TIRM, with RF                          &0.099        &0.106   &0.093 \\
  Semi segregation & STM and TIRM, with lasso                       &0.107        &0.131   &0.094 \\
  Semi segregation & TIRM only, with RF                             &0.112        &0.131   &0.094 \\
  Semi segregation & TIRM only, with lasso                          &0.127        &0.156   &0.110 \\
  Semi segregation & Word2Vec100, with lasso                        &0.217        &0.222   &0.212 \\
  \midrule

  No treatment     & STM and TIRM, with RF                               &0.271       &0.290    &0.253 \\
  No treatment     & Text tf and covariates, with lasso                  &0.310       &0.316    &0.308 \\
  No treatment     & Text tf.idf and covariates, with lasso              &0.316       &0.322    &0.312 \\
  No treatment     & Text tf.tf.idf and covariates, with lasso           &0.317       &0.324    &0.312 \\
  No treatment     & TIRM only, with RF                                  &0.318       &0.329    &0.307 \\
  \midrule

  Full segregation  & STM and TIRM, with RF                                  &0.100       &0.112   &0.0805 \\
  Full segregation  & TIRM only, with RF                                     &0.111       &0.125   &0.0841 \\
  Full segregation  & STM and TIRM, with lasso                               &0.115       &0.128   &0.0924 \\
  Full segregation  & TIRM only, with lasso                                  &0.133       &0.157   &0.105  \\
  Full segregation  & Text tf and covariates, with lasso                     &0.174       &0.185   &0.161  \\

   \bottomrule 
 \multicolumn{5}{l}{\scriptsize{Mean, max and min RMSE for each text representation overthe different folds. The 5 methods with lowest RMSE are reported.}} 
\end{tabular}
\endgroup
\caption{Ensemble learner for propensity score} 
\label{pscore.RMSE}
\end{table}


==> Tables/table_top20.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Mar 10 10:59:19 2021
\begin{table}[H]
\centering
\begingroup\scriptsize
\begin{tabular}{lllllllllllllllllllllllllllllllllllllllllllllllllllllllllllllllllllllllll}
  \toprule
BERATUNG & BERATUNG.PSYCHO & DeutschUNT & DeutschUNT.HILFE & DeutschUNT.ILZ & DeutschUNT.ISF.D\_ISF.M\_ISF & DeutschUNT.ISF.M\_ISF & DeutschUNT.KK & DeutschUNT.LOGO & DYSK & DYSK.PSYCHO & DYSK.REPETITION & Einfhrklasse & Einfhrklasse.BERATUNG & Einfhrklasse.DeutschUNT & Einfhrklasse.DeutschUNT.LOGO & Einfhrklasse.LOGO & Einfhrklasse.LOGO.PSYCHO & Einfhrklasse.PSYCHO & Einfhrklasse.PSYCHOMOT & GIFTED & GIFTED.PSYCHO & HF & HILFE & HILFE.REPETITION & ILZ & ISF & ISF.D\_ISF & ISF.D\_ISF.ILZ & ISF.D\_ISF.M\_ISF & ISF.D\_ISF.M\_ISF.REPETITION & ISF.M\_ISF & KK & KK.BERATUNG & KK.LOGO & KK.PSYCHO & KK.Zuruck & LEGA & LEGA.BERATUNG & LEGA.DYSK & LEGA.HILFE & LEGA.ISF & LEGA.ISF.D\_ISF & LEGA.ISF.M\_ISF & LEGA.KK & LEGA.LOGO & LEGA.PSYCHO & LEGA.PSYCHOMOT & LEGA.REPETITION & LOGO & LOGO.HILFE & LOGO.ISF.D\_ISF & LOGO.ISF.D\_ISF.M\_ISF & LOGO.PSYCHO & LOGO.PSYCHOMOT & LOGO.REPETITION & MULTIPLE & NONE & OTHER & PSYCHO & PSYCHO.HILFE & PSYCHO.ILZ & PSYCHO.ISF.D\_ISF & PSYCHO.ISF.D\_ISF.M\_ISF & PSYCHO.ISF.M\_ISF & PSYCHO.PSYCHOMOT & PSYCHO.REPETITION & PSYCHOMOT & REPETITION & SON & SON.LOGO & SON.PSYCHO & SON.Zuruck \\ 
  \midrule
km & ki & sr & elt & iq & math & pr & sr & sr & sr & pr & sr & sr & km & sr & pr & sr & pr & elt & ki & sr & lehr & hps & sr & lehr & shp & unterstuetz & pr & math & pr & repetition & math & sr & ki & sr & km & sr & sr & km & ki & lehr & englisch & pr & pr & sr & sr & pr & sr & repetition & sr & pr & pr & pr & dr & kiga & repetition & pr & lehr & sr & km & lehr & elt & ki & km & math & ki & gespraech & km & sr & hps & shs & mutt & sr \\ 
  mutt & km & iq & les & deutsch & kv & gespraech & iq & elt & rechn & elt & repetition & mutt & pr & iq & sr & pr & elt & mutt & km & km & pr & km & lehr & sr & mutt & ki & les & shp & math & math & km & lehr & elt & iq & sr & uebertritt & pr & lehr & km & sr & mehr & les & les & christian & pr & km & psychomotor & sr & pr & lehr & les & math & lehr & lehr & pr & km & mutt & mutt & mutt & mutt & km & km & pr & rechn & lehr & therapi & mutt & km & sr & hps & km & ki \\ 
  lehr & mutt & elt & mutt & kv & ilz & math & uebertritt & iq & lehr & km & rechn & iq & mutt & elt & iq & iq & iq & dr & mutt & elt & ergo & elt & km & pr & ilz & information & km & ilz & km & kl & pr & elt & sr & mutt & kjpd & real & les & ki & pr & mutt & macht & auswertungsgespraech & math & gross & lehr & dr & pr & rep & mutt & iq & deutsch & schwierig & mutt & sr & sr & lehr & elt & km & ki & mehr & leistung & pr & ki & lehr & schwierig & sr & ki & ki & elt & iq & hps & mutt \\ 
  sr & wenig & mutt & sprach & gemeinsam & iq & iq & gross & pr & dyskalkulietherapi & mutt & lehr & elt & mehr & emotv & elt & mutt & sr & sr & motor & lehr & sch & hpd & ki & km & pr & absprach & lehr & pr & ilz & shp & ki & iq & wenig & uebertritt & dr & wechsel & lehr & mutt & lehr & pr & re & kontextklaer & iq & iq & iq & sr & les & lehr & iq & mutt & gut & ilz & sr & abklaer & iq & sr & km & elt & sr & sr & unterstuetz & lehr & rechn & pr & abklaer & mutt & abklaer & repetition & km & kiga & sht & spd \\ 
  besprech & verhalt & pr & lehr & johanneum & pr & rechn & lehr & kram & pr & ki & rep & km & les & km & mutt & elt & gross & km & elt & pr & bess & kiga & mutt & repetition & gespraech & motti & shp & elt & iq & km & rechn & mutt & ke & lehr & el & lehr & iq & gut & sr & stuetzunterricht & pruefungsang & psychodiagnost & km & mutt & les & lehr & pmt & iq & elt & stuetzunterricht & shp & wenig & abklaer & schwierig & les & mutt & iq & ki & elt & dr & rechn & schwierig & wenig & mutt & mutt & elt & elt & elt & shs & km & dr & kg \\ 
  gespraech & math & gespraech & schwierig & sr & elt & kontextklaer & deutschunterricht & gross & mutt & dr & pr & ki & deutsch & wenig & schwierig & km & dr & iq & schwierig & bess & hawik & abklaer & stuetzunterricht & mutt & lehr & wenig & iq & iq & shp & rep & schwierig & pr & arbeit & abklaer & vb & iq & mutt & haus & rechn & les & les & gemeinsam & wenig & vgl & abklaer & elt & iq & kl & abklaer & les & auffaell & km & elt & gut & schwierig & elt & sr & pr & dr & elt & dr & kjpd & dr & iq & elt & untersuch & schwierig & iq & mutt & elt & spd & vgl \\ 
  wenig & sr & lehr & kl & gut & sgd & gemeinsam & gut & schwierig & iq & sr & kl & kram & rechn & einschul & kram & kram & mutt & abklaer & auffaell & gut & ke & einverstand & iq & real & elt & mutt & unterstuetz & rechn & rechn & pr & lehr & uebertritt & hawik & schwach & gespraech & regelklass & gut & les & rep & rechn & hawik & iq & elt & notiz & lekt & iq & auffaell & elt & km & sr & iq & iq & ki & mutt & km & schwierig & abklaer & lehr & lehr & ki & spd & dr & kjpd & kl & gespraech & besprech & lehr & pr & ki & mutt & iq & notiz \\ 
  spd & dr & gross & sr & stark & deutsch & famili & deutsch & sprach & math & lehr & iq & einschul & math & kram & einschul & einverstand & kl & pr & wenig & iq & sl & el & elt & schulisch & math & stark & gut & schreib & les & rechn & shp & gespraech & emotv & elt & iq & hawik & hawik & kv & therapi & kl & motti & motti & rechn & vereinb & auffaell & ki & wenig & hawik & gut & hawik & sprach & shp & km & elt & mutt & iq & gut & iq & gespraech & km & hawik & abklaer & schwierig & schwierig & fortschritt & evt & motor & gespraech & iv & pr & sr & hps \\ 
  emotv & lehr & deutsch & unterstuetz & lehr & wenig & psychodiagnost & rechn & deutsch & schwierig & rechn & dc-therapi & pr & ilz & pr & kg & el & k-abc & ergo & lehr & mutt & spd & schwierig & math & gespraech & spd & km & schreib & einverstand & kl & unsich & unterstuetz & einverstand & lehr & wenig & mutt & i.o & lekt & schwierig & iq & besprech & evt & gemeinsam\_auswertungsgespraech & motti & therapi & schwierig & les & k-abc & pr & auffaell & kl & sr & sprach & pr & foerder & fortschritt & ki & gespraech & gespraech & pr & ke & mutt & shp & ilz & abklaer & el & leistung & auffaell & kl & iq & sprachheilschul & elt & iq \\ 
  gut & elt & wenig & auffaell & schulisch & unterstuetz & auswertungsgespraech & elt & unterstuetz & ki & schwierig & les & schwierig & sr & einverstand & shs & lehr & wenig & schwierig & sr & dr & sj & auffaell & gespraech & mehr & iq & situation & wenig & spd & deutsch & les & iq & wenig & positiv & hawik & pr & les & elt & info & les & elt & wenig & slrt & schwierig & gut & hawik & mutt & mutt & les & schwierig & motti & unsich & deutsch & el & ilz & abklaer & math & emotv & schwierig & schwierig & situation & ergo & les & elt & emotv & ke & ke & sr & lehr & gespraech & sr & iv & iv \\ 
  pr & sl & km & deutsch & gespraech & sed & lehr & real & einschul & gut & gross & leistung & kiga & motti & ki & sprach & gross & stark & motor & pmt & kjpd & mach & mutt & pr & kl & schulrat & privat & schwierig & lernziel & ki & k-abc & mueh & km & schulisch & logop & lehr & sinnvoll & km & pr & mutt & schreib & selbstvertrau & psychodiagnost\_gemeinsam & kl & lehr & motti & hawik & seit & gut & stark & km & wenig & lehr & gut & motor & k-abc & rechn & pr & gut & kjpd & kjpd & iv & kl & mutt & gut & pmt & dr & kiga & wenig & sprachheilschul & kg & gespraech & vgl\_notiz \\ 
  neu & schwierig & rechn & re & seit & weiterfuehr & besproch & schulisch & gespraech & therapi & kjpd & schwach & einverstand & oft & lehr & wenig & einschul & schwierig & kjpd & ke & hawik & untersuch & iq & schwierig & schulrat & lernziel & kram & unsich & sr & schwierig & gross & wenig & hawik & koenn & schulleist & elt & schwach & therapi & sr & gut & iq & bemueht & kontextklaer\_psychodiagnost & hawik & uebertritt & stark & kjpd & therapi & mutt & lehr & lekt & schreib & kl & fortschritt & psychomotor & logop & les & besprech & wenig & abklaer & besprech & hochsteig & wenig & gespraech & elt & gross & el & el & mutt & weit & stark & kv & hawik \\ 
  iq & sp & les & gr & vorgespraech & diagnost & vorgespraech & leistung & gut & les & math & gut & lehr & ritalin & el & auffaell & spd & pos & lehr & fortschritt & wenig & regelklass & gespraech & kl & besprech & sr & cft & deutsch & sprach & lehr & sgd & kl & besprech & evtl & les & schwierig & rechn & rechn & mehr & el & schulrat & gross & hawik & gut & wenig & km & therapi & untersuch & unsich & fortschritt & gut & auditiv & stark & gespraech & dr & kl & wenig & el & abklaer & iq & emotv & iq & unterstuetz & math & km & schulrat & angst & wenig & einverstand & schwierig & cpm & pr & uebertritt \\ 
  kv & jedoch & einverstand & pl & schulrat & daz & norm & stark & auffaell & unsich & mehr & mueh & k-abc & bess & schwierig & spr & stark & motor & gespraech & abklaer & les & psychomotor & gross & les & geh & weit & unsich & sprach & km & unterstuetz & ilz & mutt & les & gt & einverstand & fam & psb & schreib & weg & kl & einverstand & gut & deutsch & unterstuetz & wechsel & gut & abklaer & hawik & schulisch & motti & seit & abklaer & gespraech & iq & erhalt & wenig & kl & mehr & spd & spd & real & sr & ke & iq & wenig & stark & spd & gut & shs & lehr & besuch & kg & rueckschul \\ 
  erziehungsberat & gespraech & gut & bess & red & k-abc & lektion & hawik & deutschunterricht & km & dyskalkulietherapi & math & el & cpm & kg & deutschunterricht & k-abc & motti & kispi & gespraech & emotv & iii & wenig & mehr & emotv & hawik & les & k-abc & vgl & wenig & unterstuetz & gut & el & reduziert & pr & einverstand & schwierig & ki & spd & wenig & km & mueh & shp & schreib & km & rechn & auffaell & abklaer & rechn & les & math & elt & les & kiga & les & schreib & ilz & ki & besprech & emotv & gespraech & einverstand & mehr & k-abc & les & sr & kl & pmt & rep & pr & kv & auffaell & erziehungsverantwort \\ 
  verhalt & spd & schwierig & hawik & sprachheilschul & sif & k-abc & mutt & k-abc & elt & stark & knapp & gut & diktat & deutsch & unsich & abklaer & abklaer & gut & dr & einschul & gross & gut & ke & neu & gross & aud & math & repetition & elt & deutsch & sr & kl & kaum & shs & mehr & gut & schwierig & fam & sp & repetition & pr & schulrat & lehr & zeit & mutt & schwierig & gross & motti & gross & wenig & lehr & gross & auffaell & einschul & auffaell & gespraech & spd & el & mehr & math & diethelm & kv & spd & dr & psychomotor & les & psychomotor & stao & spd & sht & fall & notiz\_vgl \\ 
  schwierig & weit & leistung & wenig & hps & standortgespraech & mutt & wenig & wenig & kl & iq & schlussbericht & wenig & gut & unsich & gut & schwierig & sprachlich & auffaell & spd & gespraech & gut & ke & gut & untersuch & vgl & hawik & sed & notiz & kv & kv & les & schwierig & haeufig & schwierig & situation & leistung & k-abc & geh & k-abc & vg & schreib & dr & jedoch & vgl\_notiz & elt & gut & unterstuetz & schwierig & kl & geht & foerder & fortschritt & gross & fortschritt & rep & gut & weit & emotv & el & abklaer & schulisch & hawik & emotv & schulisch & emotv & motti & gespraech & spd & abklaer & gespraech & shs & besprech \\ 
  ilz & stao & emotv & einverstand & st & gut & einverstand & pr & shs & gross & hawik & unsich & emotv & stark & cpm & weiterfuehr & reduziert & km & emotv & gross & mehr & abklaer & moeglich & rechn & wenig & gut & iii & hawik & vgl\_notiz & hawik & schulrat & unsich & rechn & interess & vgl & abklaer & genueg & kl & wenig & schwierig & schwierig & stark & sed & vg & hr & ki & wenig & schwierig & leistung & wenig & weiterfuehr & schwierig & rechn & shs & gross & sprachl & abklaer & hawik & dr & wenig & stuetzunterricht & gespraech & deutsch & shp & gespraech & dr & wenig & iq & dr & moeglich & gross & seit & somm \\ 
  gross & abklaer & weit & eingeschraenkt & gall & schreib & sed & mehr & cpm & hawik & kv & schulleist & unsich & sieht & gut & gross & ki & el & kram & el & el & hawik\_iii & ki & gross & kurz & geht & diktat & mueh & besprech & mutt & iq & hawik & ki & kontroll & kram & uebertritt & bereich & wenig & besproch & schulrat & spd & lehr & sgd & wld & dr & sv & el & elt & unterstuetz & kiga & schwierig & k-abc & stao & schwierig & unterstuetz & langsam & gross & wenig & kl & gut & weit & fall & math & kl & bess & km & gross & ke & les & dr & abklaer & sprachheilschul & gut \\ 
  elt & waer & schulrat & shs & st\_gall & km & gem & kaum & mueh & dc-therapi & les & mutt & abklaer & lehr & gespraech & km & unsich & seit & einschul & seit & kl & elt & sr & spd & stuetzunterricht & iv & weg & kl & unterstuetz & k-abc & elt & elt & schulrat & erziehungsberat & wechsel & ki & rueckschul & besprech & elt & ilz & math & foerder & schreib & agd & schwach & wenig & gespraech & lehr & bereich & therapeutin & allg & sed & sed & kl & pr & sprach & el & schwierig & mehr & gross & neu & v.a & el & abklaer & schreib & schulisch & abklaer & pr & hawik & kostengutsprach & ke & untersuch & elt \\ 
   \bottomrule
\end{tabular}
\endgroup
\caption{Most frequent 20 words per treatment (not ordered)} 
\label{tab:top20}
\end{table}


==> Tables/treatment.share.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Mon May 24 17:00:44 2021
\begin{table}[ht]
\centering
\begin{tabular}{llrr}
  \toprule
Variable & Treatment & Total.BROAD & Share.BROAD \\ 
  \midrule
IndTher\_BROAD & Individual therapy & 7997 & 0.509 \\ 
  ISF\_BROAD & Inclusive special ed. (ISF) & 2705 & 0.172 \\ 
  NONE\_BROAD & No therapy (but sent to SPS) & 1730 & 0.110 \\ 
  KK\_BROAD & Segr. small classes & 1690 & 0.107 \\ 
  SON\_BROAD & Segregated schooling & 1603 & 0.102 \\ 
   \bottomrule
\end{tabular}
\caption{Treatment shares} 
\end{table}

